Fully Trainable and Interpretable Non-Local Sparse Models for Image Restoration

Non-local self-similarity and sparsity principles have proven to be powerful priors for natural image modeling. We propose a novel differentiable relaxation of joint sparsity that exploits both principles and leads to a general framework for image restoration which is (1) trainable end to end, (2) fully interpretable, and (3) much more compact than competing deep learning architectures. We apply this approach to denoising, jpeg deblocking, and demosaicking, and show that, with as few as 100K parameters, its performance on several standard benchmarks is on par or better than state-of-the-art methods that may have an order of magnitude or more parameters.

==> figure_gray.tex <==

\def \1{04}
\def \2{09}
\def \3{46}
\def \4{20}
% \def \width{2.3}
% \def \Width{2.3}
\def \width{2.0}
\def \Width{2.2}


\begin{figure*}
\centering
\begin{tabular}{cccccc}
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\1_bb.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\1_gt.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\1_noise.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\1_bm3d.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\1_group.png}
	\\
	
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\2_bb.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\2_gt.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\2_noise.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\2_bm3d.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\2_group.png}
	\\	
	
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\3_bb.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\3_gt.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\3_noise.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\3_bm3d.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\3_group.png}
	\\
	
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bb.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_gt.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_noise.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bm3d.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_group.png}
%	\\
	\begin{tabular}{cc}Original image\\ and close-up region  \end{tabular}&
	 Ground truth &
	\begin{tabular}{cc}Noisy image\\ $\sigma=25$  \end{tabular}&
	BM3D & 
	\begin{tabular}{cc}\textbf{GroupSC}\\ \textbf{(ours)} \end{tabular} \\
\end{tabular}
\caption{Grey denoising results for 3 images from the BSD68 dataset.Best seen
by zooming on a computer screen.}	\label{fig:color}

%\vspace*{-1cm}
\end{figure*}

==> latexSource (copy)/abstract.tex <==
Non-local self-similarity and sparsity principles have proven to be 
powerful priors for natural image modeling. We propose a novel 
differentiable relaxation of joint sparsity that exploits both 
principles and leads to a general framework for image restoration which 
is (1) trainable end to end, (2) fully interpretable, and (3) much more 
compact than competing deep learning architectures. We apply this 
approach to denoising, blind denoising, jpeg deblocking, and demosaicking, and show that, 
with as few as 100K parameters, its performance on several standard 
benchmarks is on par or better than state-of-the-art methods that may 
have an order of magnitude or more parameters.


==> latexSource (copy)/conclusion.tex <==
We have presented a differentiable algorithm based on non-local sparse image
models, which performs on par or better than recent deep learning models, while
using significantly less parameters.  We believe that the performance of such
approaches---including the simple SC baseline---is surprising given the small
model size, and given the fact that the algorithm can be interpreted as a
single sparse coding layer operating on fixed-size patches.
This observation paves the way for future work for sparse coding models that should 
be able to model the local stationarity of natural images at multiple scales,
which we expect should perform even better.
We believe that our work also confirms that model-based image restoration principles  
developed about a decade ago are still useful to improve current deep learning models 
and are a key to push their current limits.


==> latexSource (copy)/demosaicking.tex <==
Most modern digital cameras acquire color images by measuring only one color
channel per pixel, red, green, or blue, according to a specific pattern called
the Bayer pattern.  Demosaicking is the processing step that reconstruct a full
color image given these incomplete measurements. 

Originally addressed by using interpolation techniques~\cite{gunturk},
demosaicking has been successfully tackled by
sparse coding~\cite{mairal2009non} and deep learning models.
Most of them such as \cite{zhang2017learning,zhang2019rnan} rely on generic
architectures and black box models that do not encode a priori knowledge about the 
problem, whereas the authors of \cite{kokkinos2019iterative} 
propose an iterative algorithm that relies on the physics of the acquisition process.
Extending our model to demosaicking (and in fact to other inpainting tasks with small holes)
can be achieved by introducing a mask~$\Mb_i$ in the formulation for unobserved pixel values.
Formally we define $\Mb_i$ for patch $i$ as a vector in $\{0,1\}^{m}$, and $\Mb = [\Mb_0, \dots, \Mb_N]$ in $\{0,1\}^{n\times N}$ represents all masks. 
Then, the sparse coding formulation becomes
\begin{equation} \label{mosaic_optim}
\min_{\Ab} \frac{1}{2} \| \Mb \odot (\Yb^c-\Db \Ab)\|_{\text{F}}^2 + \sum_{i=1}^N \Psi_i(\Ab),
\end{equation}
where $\odot$ denotes the elementwise product between two matrices.  The first updating rule of equation~(\ref{eq:lista_group}) is modified accordingly. This lead to a different update which has the effect of discarding reconstruction error of masked pixels,
\begin{equation}
   \Bb  \leftarrow \Ab^{(k)} +  \Cb^\top (\Mb \odot (\Yb^c-\Db\Ab^{(k)})). 
\end{equation}




==> latexSource (copy)/experiments_eccv.tex <==


\paragraph{Training details and datasets.} In our experiments, we adopt the
setting of \cite{zhang2017beyond}, which is the most standard one used by
recent deep learning methods, allowing a simple and fair comparison.  In
particular, we use as a training set a subset of the Berkeley Segmentation
Dataset (BSD) \cite{martin2001database}, called BSD400.
We evaluate our models on 3 popular benchmarks: BSD68 (with no overlap with BSD400), Kodak24, and Urban100  \cite{huang2015single} and on Classic5 for Jpeg deblocking, following \cite{foi2007pointwise,yu2016deep}.
For gray denoising and Jpeg deblocking  we choose a patch size of $9\times9$ and dictionary with 256 atoms for our models, whereas we choose a patch size of  $7\times7$ for color denoising and demosaicking.
 For all our experiments, we randomly extract patches of size $56\times56$ whose size equals the neighborhood for non-local operations and optimize the parameters of our models using ADAM~\cite{kingma2014adam}.  Similar to \cite{simon2019rethinking}, we normalize the initial dictionnary $\Db_0$ by its largest singular value, which helps the LISTA algorithm to converge. We also implemented a backtracking strategy that automatically decreases the learning rate by a factor 0.5 when the training loss diverges.
Additional training details can be found in the appendix for reproductibility purposes.

\vsp
\paragraph{Performance measure.} We use the PSNR as a quality measure, but SSIM scores for our experiments are provided in the appendix, leading to similar conclusions.

\vsp
\paragraph{Grayscale Denoising.}
We train our models under the same setting as \cite{zhang2017beyond,lefkimmiatis2017non,liu2018non}. We corrupt images with synthetic additive gaussian noise with a variance $\sigma = \{5,15,25,50 \}$ and train a different model for each~$\sigma$ and report the performance in terms of PSNR. 
Our method appears to perform on par with DnCNN for $\sigma \geq 10$ and performs significantly better for low-noise settings. Finaly we  provide results on other datasets in the appendix. 
On BSD68 the light version of our method runs 10 times faster than NLRN \cite{liu2018non} (2.17s for groupSC and 21.02s for NLRN), see the appendix for detailed experiments concerning the running time our our method ans its variants.

\vsp
\paragraph{Color Image Denoising}
We train our models under the same setting as \cite{lefkimmiatis2017non,zhang2017beyond}; we corrupt images with synthetic additive gaussian noise with a variance $\sigma = \{5,10,15,25,30,50\} $ and we train a different model for each variance of noise. 
%We choose a patch size of $7\times7$ and set the size of the dictionary to 256.
%
For reporting both qualitative and quantitative results of {BM3D-PCA} \cite{dabov2009bm3d} and {DnCNN} \cite{zhang2017beyond} we used the implementation realeased by the authors. For the other methods we provide the numbers reported in the corresponding papers.
%
We report the performance of our model in Table \ref{colour_table} and report qualitative results in Figure~\ref{fig:color}, along with those of competitive approaches, and provide results on other datasets in the appendix. 
%Finally, we compare our model with \cite{zhang2019rnan} in Table \ref{colour_table_rnan} for $\sigma=10,30$ because we did not manage to run their code for the sigma values considered in Table~\ref{colour_table}.
Overall, it seems that RNAN performs slightly better than GroupSC, at a cost of using $76$ times more parameters.

\vsp
\paragraph{Blind Color Image Denoising.}
We compare our model with \cite{lefkimmiatis2018universal,zhang2017beyond,dabov2009bm3d} and report our results in Table \ref{tab:blind}. \cite{lefkimmiatis2018universal} trains two different models in the range [0,25] and [25,50]. We compare with their model trained in the range [0,25] for a fair comparaison. We use the same hyperparameters than the one used for color denoising experiments. Our model performs consistently better than other methods.

\vsp
\paragraph{Demosaicking.} \label{section_expe_mosaic}
We follow the same experimental setting as IRCNN \cite{zhang2017learning}, but we do not crop the output images similarly to \cite{zhang2017learning,mairal2009non} since \cite{zhang2019rnan} does not seem to perform such an operation according to their code online. We compare our model with sate-of-the-art deep learning methods \cite{kokkinos2018deep,kokkinos2019iterative,zhang2019rnan} and also report the performance of LSSC.  
% 
For the concurrent methods we provide the numbers reported in the corresponding papers. 
On  BSD68, the light version of our method(groupsc) runs at about the same speed than RNAN for demosaicking (2.39s for groupsc and 2.31s for RNAN).
We observe that our baseline provides already very good results, which is surprising given its simplicity, but suffers from more visual artefacts than GroupSC (see Fig. \ref{fig:mosaic}). Compared to RNAN, our model is much smaller
and shallower (120 layers for RNAN and 24 iterations for ours). We also note that CSR performs poorly in comparison with groupSC. 

\vsp
\paragraph{Compression artefacts reduction.}
For jpeg deblocking, we compare our approach with
state-of-the-art methods using the same experimental setting: we only
restore images in the Y channel (YCbCr space) and train our models on
the CBSD400 dataset. Our model performs consistently better than other approaches.



==> latexSource (copy)/fig_mosa.tex <==
% \begin{figure*}[t]
% \def \width{2.3}
% \centering
% \begin{tabular}{ccccc}
% \includegraphics[width=\width cm]{figures/mosa/70_sc.png} & 
% \includegraphics[width=\width cm]{figures/mosa/60_sc.png} &
% \includegraphics[width=\width cm]{figures/mosa/88_sc.png} & 
% \includegraphics[width=\width cm]{figures/mosa/66_sc.png}&
% \includegraphics[width=\width cm]{figures/mosa/24_sc.png}

% \\
% \includegraphics[width=\width cm]{figures/mosa/70_group.png} & 
% \includegraphics[width=\width cm]{figures/mosa/60_group.png}&
% \includegraphics[width=\width cm]{figures/mosa/88_group.png} & 
% \includegraphics[width=\width cm]{figures/mosa/66_group.png}&
% \includegraphics[width=\width cm]{figures/mosa/24_group.png}

% \\
% \end{tabular}
% \caption{\textbf{Demosaicking}. Top: reconstructions with sparse prior only, exhibiting classical artefacts. Bottom: reconstruction with both priors, artefact-free. The figure should be seen in color.}
% \label{fig:supp_mosa}
%   \vspace*{-0.4cm}
% \end{figure*}


\def \1{23}
\def \2{14}
\def \3{07}
\def \4{20}
% \def \width{2.3}
% \def \Width{2.3}
\def \width{2.0}
\def \Width{1.9}


%\begin{figure*}
%\centering
%\begin{tabular}{cccccc}
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_bb.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_gt.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_noise.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_bm3d.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_dn.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_group.png}
%	\\
%	
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_bb.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_gt.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_noise.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_bm3d.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_dn.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_group.png}
%	\\	
%	
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_bb.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_gt.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_noise.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_bm3d.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_dn.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_group.png}
%	\\
%	
%%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bb.png}&
%%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_gt.png}&
%%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_noise.png}&
%%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bm3d.png}&
%%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_group.png}
%%	\\
%	\begin{tabular}{cc}Original image\\ and close-up region  \end{tabular}&
%	 Ground truth &
%	\begin{tabular}{cc}Noisy image\\ $\sigma=25$  \end{tabular}&
%	CBM3D & 
%	CDnCNN &
%	\begin{tabular}{cc}\textbf{GroupSC}\\ \textbf{ours} \end{tabular} \\
%\end{tabular}
%\end{figure*}

\def \1{60}
\def \2{70}
\def \3{92}
\def \4{26}
% \def \width{2.3}
% \def \Width{2.3}
\def \width{2.5}
\def \Width{1.9}

\begin{figure*}[h!]
\centering
\begin{tabular}{cccccc}
	\includegraphics[width=\Width cm]{figures/mosa_app/\1_bb.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\1_gt.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\1_noise.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\1_sc.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\1_ircnn.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\1_group.png}
	\\
    \includegraphics[width=\Width cm]{figures/mosa_app/\2_bb.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\2_gt.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\2_noise.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\2_sc.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\2_ircnn.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\2_group.png}
	\\
    \includegraphics[width=\Width cm]{figures/mosa_app/\3_bb.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\3_gt.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\3_noise.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\3_sc.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\3_ircnn.png}&
	\includegraphics[width=\Width cm]{figures/mosa_app/\3_group.png}
    \\

    Original image &	
	Ground truth &
	Corrupted&
	SC & 
	IRCNN &
	\begin{tabular}{cc}\textbf{GroupSC}\\ \textbf{(ours)} \end{tabular} \\
\end{tabular}
\vspace*{-0.4cm}

\caption{Color denoising results for 3 images from the Urban100 dataset. Best seen in color
by zooming on a computer screen. On the three images, our approach groupSC exhibits significantly less artefacts than IRCNN and our baseline SC.}	\label{fig:supp_mosa}

\end{figure*}


==> latexSource (copy)/figure_color_app.tex <==

\def \1{12}
\def \2{15}
\def \3{06}
\def \4{07}
% \def \width{2.3}
% \def \Width{2.3}
\def \width{2.0}
\def \Width{1.9}


%\begin{figure*}
%\centering
%\begin{tabular}{cccccc}
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_bb.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_gt.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_noise.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_bm3d.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_dn.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\1_group.png}
%	\\
%	
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_bb.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_gt.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_noise.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_bm3d.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_dn.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\2_group.png}
%	\\	
%	
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_bb.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_gt.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_noise.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_bm3d.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_dn.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\3_group.png}
%	\\
%	
%%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bb.png}&
%%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_gt.png}&
%%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_noise.png}&
%%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bm3d.png}&
%%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_group.png}
%%	\\
%	\begin{tabular}{cc}Original image\\ and close-up region  \end{tabular}&
%	 Ground truth &
%	\begin{tabular}{cc}Noisy image\\ $\sigma=25$  \end{tabular}&
%	CBM3D & 
%	CDnCNN &
%	\begin{tabular}{cc}\textbf{GroupSC}\\ \textbf{ours} \end{tabular} \\
%\end{tabular}
%\end{figure*}

\begin{figure*}[h!]
\centering
\begin{tabular}{ccccccc}
% 	\includegraphics[width=\Width cm]{figures/color_denoising/\1_bb.png}&
% 	\includegraphics[width=\Width cm]{figures/color_denoising/\1_gt.png}&
% 	\includegraphics[width=\Width cm]{figures/color_denoising/\1_noise.png}&
% 	\includegraphics[width=\Width cm]{figures/color_denoising/\1_bm3d.png}&
% 			\includegraphics[width=\Width cm]{figures/color_denoising/\1_dn.png}&
% 	\includegraphics[width=\Width cm]{figures/color_denoising/\1_group.png}
% 	\\
	
	\includegraphics[width=\Width cm]{figures/color_denoising/\2_bb.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\2_gt.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\2_noise.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\2_bm3d.png}&
			\includegraphics[width=\Width cm]{figures/color_denoising/\2_dn.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\2_group.png}
	\\	
	
	\includegraphics[width=\Width cm]{figures/color_denoising/\3_bb.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\3_gt.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\3_noise.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\3_bm3d.png}&
		\includegraphics[width=\Width cm]{figures/color_denoising/\3_dn.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\3_group.png}
	\\

	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bb.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\4_gt.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\4_noise.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bm3d.png}&
		\includegraphics[width=\Width cm]{figures/color_denoising/\4_dn.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\4_group.png}
	\\
%	
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bb.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_gt.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_noise.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bm3d.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_group.png}
%	\\
%	\begin{tabular}{cc}Original image\\ \& close-up region  \end{tabular}&
Original image &	
	 Ground truth &
	\begin{tabular}{cc}Noisy image\\ $\sigma=25$  \end{tabular}&
	CBM3D & 
	CDnCNN &
	\begin{tabular}{cc}\textbf{GroupSC}\\ \textbf{(ours)} \end{tabular} \\
\end{tabular}
% \vspace*{-0.4cm}

\caption{Color denoising results for 3 images from the Kodak24 dataset. Best seen in color
   by zooming on a computer screen. Artefact reduction compared to CDnCNN can be seen in the top and bottom pictures (see in particular the flower's pistil).}	\label{fig:supp_color}

\end{figure*}


==> latexSource (copy)/figure_colore.tex <==

\def \1{23}
\def \2{14}
\def \3{_07}
\def \4{20}

\def \width{2.0}
\def \Width{1.9}

\begin{figure*}[h]
\centering
\begin{tabular}{ccccccc}
	\includegraphics[width=\Width cm]{figures/color_denoising/\1_bb.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\1_gt.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\1_noise.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\1_bm3d.png}&
			\includegraphics[width=\Width cm]{figures/color_denoising/\1_dn.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\1_group.png}
	\\
	
	\includegraphics[width=\Width cm]{figures/color_denoising/\2_bb.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\2_gt.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\2_noise.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\2_bm3d.png}&
			\includegraphics[width=\Width cm]{figures/color_denoising/\2_dn.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\2_group.png}
	\\	
	
	\includegraphics[width=\Width cm]{figures/color_denoising/\3_bb.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\3_gt.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\3_noise.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\3_bm3d.png}&
		\includegraphics[width=\Width cm]{figures/color_denoising/\3_dn.png}&
	\includegraphics[width=\Width cm]{figures/color_denoising/\3_group.png}
	\\

Original image &	
	 Ground truth &
	\begin{tabular}{cc}Noisy image\\ $\sigma=25$  \end{tabular}&
	CBM3D & 
	CDnCNN &
	\begin{tabular}{cc}\textbf{GroupSC}\\ \textbf{(ours)} \end{tabular} \\
\end{tabular}
% \vspace*{-0.4cm}

\caption{Color denoising results for 3 images from the Kodak24 dataset. Best seen in color
by zooming on a computer screen. More qualitative results for other tasks are in appendix.}	\label{fig:color}

\end{figure*}


==> latexSource (copy)/figure_gray.tex <==

\def \1{04}
\def \2{09}
\def \3{46}
\def \4{20}
% \def \width{2.3}
% \def \Width{2.3}
\def \width{2.0}
\def \Width{2.2}


\begin{figure*}
\centering
\begin{tabular}{cccccc}
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\1_bb.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\1_gt.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\1_noise.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\1_bm3d.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\1_group.png}
	\\
	
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\2_bb.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\2_gt.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\2_noise.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\2_bm3d.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\2_group.png}
	\\	
	
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\3_bb.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\3_gt.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\3_noise.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\3_bm3d.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/g\3_group.png}
	\\
	
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bb.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_gt.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_noise.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_bm3d.png}&
%	\includegraphics[width=\Width cm]{figures/color_denoising/\4_group.png}
%	\\
	\begin{tabular}{cc}Original image\\ and close-up region  \end{tabular}&
	 Ground truth &
	\begin{tabular}{cc}Noisy image\\ $\sigma=25$  \end{tabular}&
	BM3D & 
	\begin{tabular}{cc}\textbf{GroupSC}\\ \textbf{(ours)} \end{tabular} \\
\end{tabular}
\caption{Grey denoising results for 3 images from the BSD68 dataset.Best seen
by zooming on a computer screen.}	\label{fig:color}

%\vspace*{-1cm}
\end{figure*}

==> latexSource (copy)/figure_gray_app.tex <==

\def \1{g011}
\def \2{g006}
\def \3{g020}
\def \4{g23}


\def \width{2.0}
\def \Width{1.9}



\begin{figure*}[h!]
\centering
\begin{tabular}{cccccc}
	\includegraphics[width=\Width cm]{figures/gray_denoising/\1_bb.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\1_gt.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\1_noise.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\1_bm3d.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\1_dn.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\1_group.png}
	\\
	
	\includegraphics[width=\Width cm]{figures/gray_denoising/\2_bb.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\2_gt.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\2_noise.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\2_bm3d.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\2_dn.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\2_group.png}
	\\	
%     \includegraphics[width=\Width cm]{figures/gray_denoising/\3_bb.png}&
% 	\includegraphics[width=\Width cm]{figures/gray_denoising/\3_gt.png}&
% 	\includegraphics[width=\Width cm]{figures/gray_denoising/\3_noise.png}&
% 	\includegraphics[width=\Width cm]{figures/gray_denoising/\3_bm3d.png}&
% 	\includegraphics[width=\Width cm]{figures/gray_denoising/\3_dn.png}&
% 	\includegraphics[width=\Width cm]{figures/gray_denoising/\3_group.png}
% 	\\	
	\includegraphics[width=\Width cm]{figures/gray_denoising/\4_bb.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\4_gt.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\4_noise.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\4_bm3d.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\4_dn.png}&
	\includegraphics[width=\Width cm]{figures/gray_denoising/\4_group.png}
	\\	
    Original image &	
    Ground truth &
   \begin{tabular}{cc}Noisy image\\ $\sigma=25$  \end{tabular}&
   BM3D & 
   DnCNN &
   \begin{tabular}{cc}\textbf{GroupSC}\\ \textbf{(ours)} \end{tabular} \\
\end{tabular}
\vspace*{-0.4cm}


\caption{Grey denoising results for 3 images from the BSD68 dataset. Best seen 
by zooming on a computer screen. GroupSC's images are slightly more detailed than DnCNN on the top and middle image, whereas DnCNN does subjectively slightly better on the bottom one. Overall, these two approaches perform similarly on this dataset.}	\label{fig:supp_gray}

\end{figure*}


==> latexSource (copy)/figure_jpeg.tex <==

\def \1{barbara}
\def \2{lena}
\def \3{baboon}


\def \width{1.8}
\def \Width{1.75}



\begin{figure*}[h!]
\centering
\begin{tabular}{cccccc}
	\includegraphics[width=\Width cm]{figures/jpeg/\1_bb.png}&
	\includegraphics[width=\Width cm]{figures/jpeg/\1_gt.png}&
    \includegraphics[width=\Width cm]{figures/jpeg/\1_noisy.png}&
    \includegraphics[width=\Width cm]{figures/jpeg/\1_arcnn.png}&
	\includegraphics[width=\Width cm]{figures/jpeg/\1_sc.png}&
	\includegraphics[width=\Width cm]{figures/jpeg/\1_group.png}
	\\
	
	\includegraphics[width=\Width cm]{figures/jpeg/\2_bb.png}&
	\includegraphics[width=\Width cm]{figures/jpeg/\2_gt.png}&
    \includegraphics[width=\Width cm]{figures/jpeg/\2_noisy.png}&
    \includegraphics[width=\Width cm]{figures/jpeg/\2_arcnn.png}&
	\includegraphics[width=\Width cm]{figures/jpeg/\2_sc.png}&
			% \includegraphics[width=\Width cm]{figures/jpeg/\2_dn.png}&
	\includegraphics[width=\Width cm]{figures/jpeg/\2_group.png}
	\\	
	\includegraphics[width=\Width cm]{figures/jpeg/\3_bb.png}&
	\includegraphics[width=\Width cm]{figures/jpeg/\3_gt.png}&
    \includegraphics[width=\Width cm]{figures/jpeg/\3_noisy.png}&
    \includegraphics[width=\Width cm]{figures/jpeg/\3_arcnn.png}&
	\includegraphics[width=\Width cm]{figures/jpeg/\3_sc.png}&
	\includegraphics[width=\Width cm]{figures/jpeg/\3_group.png}
	\\
Original image &	
	 Ground truth &
    Jpeg&
    ARCNN&
    SC (ours) &
	\begin{tabular}{cc}\textbf{GroupSC}\\ \textbf{(ours)} \end{tabular} \\
\end{tabular}
\vspace*{-0.4cm}
\caption{Jpeg artefact reduction results for 2 images from the Classic5 dataset. Best seen in color
by zooming on a computer screen.}	\label{fig:supp_jpeg}


\end{figure*}


==> latexSource (copy)/intro.tex <==
 

The image processing community has long focused on designing
 handcrafted models of natural images to address inverse problems,
leading, for instance, to  
differential operators~\cite{perona1990}, total
variation~\cite{rudin1992nonlinear}, or wavelet sparsity~\cite{mallat} approaches. More recently,
image restoration para\-digms have shifted towards data-driven
approaches. For instance, non-local
means~\cite{buades2005non} exploits self-similarities, 
and many successful approaches have relied on
unsupervised methods such as learned sparse models~\cite{aharon2006k,mairal2014sparse},
Gaussian scale mixtures~\cite{portilla}, or fields of experts~\cite{roth}.
More powerful models such as BM3D~\cite{dabov2009bm3d} have also been obtained by combining several priors, in particular self-similarities and sparse
representations 
\cite{dabov2007image,dabov2009bm3d,dong2012nonlocally,gu2014weighted,mairal2009non}.

These methods are now often outperformed by
deep learning models, which are able to leverage pairs of corrupted/clean
images for supervised learning,
in  tasks such as
denoising~\cite{lefkimmiatis2017non,liu2018non,plotz2018neural,zhang2017beyond},
demoisaicking~\cite{kokkinos2019iterative,zhang2017learning,zhang2019rnan},
upsampling~\cite{dong2015image,kim2016accurate}, or artefact removal~\cite{zhang2019rnan}.  Yet, they also suffer from lack of
interpretability and the need to learn a huge number of parameters.
Improving these two aspects is
one of the key motivation of this paper.  Our goal is to design algorithms that bridge the gap in performance between earlier approaches
that are parameter-efficient and interpretable, and current deep
models. 

Specifically, we propose a differentiable relaxation of the non-local sparse
model LSSC~\cite{mairal2009non}. 
The relaxation allows us to obtain models that may be trained end-to-end,
and which admit a simple interpretation in terms of joint sparse coding
of similar patches.
The principle of end-to-end training for sparse coding was
introduced in~\cite{mairal2011task}, and later combined in~\cite{wang2015deep} for super-resolution
with variants of the LISTA
algorithm~\cite{chen2018theoretical,gregor2010learning,liu2018alista}.
A variant based on convolutional sparse coding was then proposed
in~\cite{simon2019rethinking} for image denoising, and another one based on
the K-SVD algorithm~\cite{elad2006image} was introduced in~\cite{scetbon2019deep}.
Note that these works are part of a vast litterature on model-inspired methods,
 where the model architecture is related to an optimization strategy for minimizing an objective,
  see~\cite{lefkimmiatis2017non,sun2016deep,venkatakrishnan2013plug}. 

In contrast, our main contribution is to extend the idea of differentiable
algorithms to \emph{structured} sparse models~\cite{jenatton2011structured},
which is a key concept behind the LSSC, CSR, and BM3D approaches.
To the best of our knowledge, this is the first time that non-local sparse
models are shown to be effective in a supervised learning setting.
As~\cite{scetbon2019deep}, we argue that bridging classical successful image
priors within deep learning frameworks is a key to overcome the limitations of
current state-of-the-art models.  A striking fact is notably the performance of 
the resulting models given their low number of parameters. 

For example, our method for image denoising performs on par with the
deep learning baseline DnCNN~\cite{zhang2017beyond} with $8$x less
parameters, significantly outperforms the color variant CDnCNN with $6$x
less parameters, and achieves state-of-the-art results for blind
denoising and jpeg deblocking. 
For these two last tasks, relying on an interpretable model is important;
most parameters are devoted to image reconstruction and can be shared 
by models dedicated to different noise levels. Only a small subset of parameters can be
seen as regularization parameters, and may be made noise-dependent,
thus removing the burden of training several large independent models for each noise level.
For image demosaicking, we obtain similar results
as the state-of-the-art approach RNAN~\cite{zhang2019rnan}, while reducing the
number of parameters by $76$x.
Perhaps more important than improving the PSNR, the
principle of non local sparsity also reduces visual artefacts when compared to
using sparsity alone,
which is illustrated in Figure~\ref{fig:mosaic}.

Our models are implemented in PyTorch and our code can be found at \url{ https://github.com/bruno-31/groupsc}.


==> latexSource (copy)/macros.tex <==
\newcommand\vsp{\vspace*{-0.0cm}}
\newcommand\yb{\mathbf{y}}
\newcommand\Yb{\mathbf{Y}}
\newcommand\xb{\mathbf{x}}
\newcommand\Db{\mathbf{D}}
\newcommand\Ab{\mathbf{A}}
\newcommand\Ub{\mathbf{U}}
\newcommand\Zb{\mathbf{Z}}
\newcommand\ub{\mathbf{u}}
\newcommand\wb{\mathbf{w}}
\newcommand\zb{\mathbf{z}}
\newcommand\Cb{\mathbf{C}}
\newcommand\Ib{\mathbf{I}}
\newcommand\Wb{\mathbf{W}}
\newcommand\Rb{\mathbf{R}}
\newcommand\Mb{\mathbf{M}}
\newcommand\Bb{\mathbf{B}}
\newcommand\db{\mathbf{d}}

\newcommand\ones{\mathbf{1}}
\newcommand\Real{\mathbb{R}}
\newcommand\alphab{\boldsymbol{\alpha}}
\newcommand\betab{\boldsymbol{\beta}}
\newcommand\Lambdab{\boldsymbol{\Lambda}}
\newcommand\Thetab{\boldsymbol{\Theta}}
\newcommand\Sigmab{\boldsymbol{\Sigma}}
\newcommand\kappab{\boldsymbol{\kappa}}

\newcommand\Pcal{{\mathcal{P}}}



==> latexSource (copy)/method.tex <==

We now present trainable sparse coding models for image denoising,
following~\cite{simon2019rethinking}, with a few minor improvements,
before introducing differentiable relaxations for the LSSC method \cite{mairal2009non} .
% We also introduce relaxations for CSR in the appendix.
%
A different approach to take into account self similarities in sparse models is
the CSR approach \cite{dong2012nonlocally}. We have
empirically observed that it does not perform as well as LSSC. Nevertheless, we believe it to be
conceptually interesting, and provide a brief description in the appendix.

\subsection{Trainable Sparse Coding (without Self-Similarities)}\label{subsec:sc}
In \cite{simon2019rethinking}, the sparse coding approach (SC) is combined with the LISTA algorithm to perform
denoising tasks.\footnote{Specifically, \cite{simon2019rethinking} proposes a model based on
   convolutional sparse coding (CSC).
   CSC is a variant of SC, where a full image is
   approximated by a linear combination of small dictionary elements. Unfortunately, CSC leads to
   ill-conditioned optimization problems and has shown to perform poorly
   for image denoising.  For this reason,~\cite{simon2019rethinking} introduces
   a hybrid approach between SC and CSC.
   In our paper, we have decided to use the SC baseline and leave the investigation of CSC models for
   future work.}
The only modification we introduce here is a centering step
for the patches, which empirically yields better results.

\begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/fig1_c.pdf}
   \caption{An illustration of the main inference algorithm for GroupSC.
      See Figure \ref{fig:nlmodule} for an illustration of the self-similarity module.}\label{fig:diagram}
\end{figure}

\begin{figure}[t] 
   \centering
   \includegraphics[width=0.80\linewidth]{figures/fig2_c.pdf}
   \caption{An illustration of the self-similarity module used in our GroupSC algorithm.}\label{fig:nlmodule}
\end{figure}

\vsp
\paragraph{SC Model - inference with fixed parameters.}
%We now explain how an input image $\yb$ is represented in the SC model, before discussing how to learn the parameters. 
Following the approach and notation from Section~\ref{sec:related},
the first step consists of extracting all overlapping patches $\yb_1,\ldots,\yb_n$. %= \mathcal{T}(\yb)$, where $\mathcal{T}$ is a linear patch extraction operator.  
Then, we perform the centering operation for every patch
\begin{equation}
   \yb_i^{c} \triangleq \yb_i - \mu_i \ones_m ~~~\text{with}~~~~ \mu_i \triangleq \frac{1}{m} \ones_m^\top  \yb_i.\label{eq:centering}
\end{equation}
The mean value~$\mu_i$ is recorded and added back after denoising $\yb_i^c$. Hence,
low-frequency components do not flow through the model.
The centering step is not used in~\cite{simon2019rethinking}, but we have
found it to be useful. %provide better reconstruction quality.

The next step consists of sparsely encoding each centered patch $\yb_i^c$ with
$K$ steps of the LISTA variant presented in~(\ref{eq:recurrent}), replacing $\yb_i$
by $\yb_i^c$ there, assuming the parameters $\Db, \Cb$ and $\Lambdab_{k}$ are
given.
Here, a minor change compared to~\cite{simon2019rethinking}
is the use of varying parameters $\Lambdab_{k}$ at each LISTA step. %,
Finally, the final image is obtained by averaging the patch estimates as in~(\ref{eq:averaging}),
after adding back $\mu_i$:
\begin{equation}
   \hat{\xb} = \frac{1}{n} \sum_{i=1}^N \Rb_i (\Wb \alphab_i^{(K)} + \mu_i \ones_m), \label{eq:averaging2}
\end{equation}
but the dictionary~$\Db$ is replaced by another matrix~$\Wb$.
The reason for decoupling $\Db$ from $\Wb$ is that the $\ell_1$ penalty used by the LISTA method is known to shrink the coefficients~$\alphab_i$
too much.
For this reason, classical
denoising approaches such as~\cite{elad2006image,mairal2009non} use instead the $\ell_0$-penalty,
but we have found it ineffective for
end-to-end training. Therefore, as in~\cite{simon2019rethinking},
we have chosen
to decouple $\Wb$ from~$\Db$.

\vsp
\paragraph{Training the parameters.}

We now assume that we are given a training set of pairs of
clean/noisy images $(\xb,\yb) \sim \Pcal$, and we minimize in a supervised fashion
\begin{equation}
   \min _{\Thetab}  \EX_{(\xb,\yb) \sim \Pcal}  \left\| \hat{\xb}(\yb) - \xb\right\|_2^2,\label{eq:cost}
\end{equation}
where $\Thetab =
   \{\Cb,\Db,\Wb,(\Lambdab_{k})_{k=0,1 \dots K-1}, \kappab, \nu \}$ is the set of parameters to learn and $\hat{\xb}$ is the denoised image defined in~(\ref{eq:averaging2}).

\subsection{Differentiable Relaxation for Non-Local Sparse Priors}
\begin{algorithm}
   \caption{Pseudo code for the inference model of GroupSC.}\label{alg:pseudo}
   \begin{algorithmic}[1]
      \State Extract patches $\Yb=[\yb_1,\ldots,\yb_n]$ and center them with~(\ref{eq:centering});
      \State Initialize the codes $\alphab_i$ to $0$;
      \State Initialize image estimate $\hat{\xb}$ to the noisy input $\yb$;
      \State Initialize pairwise similarities~$\Sigmab$ between patches of $\hat{\xb}$;
      \For {$k=1,2,\ldots K$}
      \State Compute pairwise patch similarities~$\hat{\Sigmab}$ on~$\hat{\xb}$;
      \State Update $\Sigmab \leftarrow (1-\nu) \Sigmab + \nu \hat{\Sigmab}$;
      \For {$i=1,2,\ldots,N$ in parallel}
      \State $\alphab_i \leftarrow \prox_{\Sigmab, \Lambdab_k} \left [\alphab_i+ \Cb^\top(\yb_i^c-\Db\alphab_i) \right]$;
      \EndFor
      \State Update the denoised image~$\hat{\xb}$ by averaging~(\ref{eq:averaging2});
      \EndFor
   \end{algorithmic}
\end{algorithm}

Self-similarities are modeled by replacing the $\ell_1$-norm by
structured sparsity-inducing regularization functions. In Algorithm~\ref{alg:pseudo}, we
present a generic approach to use this principle within a supervised learning approach,
based on a similarity matrix $\Sigmab$,
overcoming the difficulty of hard clustering/grouping patches together. In Figure~\ref{fig:diagram}, we also provide a diagram of one step of the inference algorithm.
At each step, the method computes pairwise patch similarities~$\Sigmab$
between patches of a current estimate~$\hat{\xb}$, using various possible
metrics that we discuss in Section~\ref{sec:similarities}.
The codes~$\alphab_i$ are updated by computing a so-called proximal operator, defined below, for a particular
penalty that depends on $\Sigmab$ and some parameters $\Lambdab_k$. Practical variants
where the pairwise similarities are only updated once in a while, are discussed in Section~\ref{sec:extensions}.
\begin{definition}[Proximal operator]
   Given a convex function~$\Psi: \Real^p \!\to\! \Real$, the proximal operator of $\Psi$ is defined~as the unique solution of
   \begin{equation}
      \prox_{\Psi}[\zb] = \argmin_{\ub \in \Real^p} \frac{1}{2}\|\zb-\ub\|^2 + \Psi(\ub).
   \end{equation}
\end{definition}
The proximal operator plays a key role in optimization and admits a closed form
for many penalties, see~\cite{mairal2014sparse}.
Indeed, given~$\Psi$, it may be shown that the iterations
$\alphab_i \leftarrow \prox_{\eta\Psi} \left [\alphab_i+ \eta \Db^\top(\yb_i^c-\Db\alphab_i) \right]$
are instances of the ISTA algorithm~\cite{beck2009fast} for minimizing
$$ \min_{\alphab_i \in \Real^p} \frac{1}{2}\|\yb_i^c - \Db\alphab_i\|^2 + \Psi(\alphab_i),$$
and the update of $\alphab_i$ in Algorithm~\ref{alg:pseudo} simply extend LISTA to deal with~$\Psi$.
Note that for the weighted $\ell_1$-norm $\Psi(\ub) = \sum_{j=1}^p \lambda_j \left | \ub[j]  \right | $, the proximal operator is the soft-thresholding
operator $S_{\Lambda}$ introduced in Section~\ref{sec:related} for $\Lambdab = (\lambda_1,\ldots,\lambda_p)$ in $\Real^p$,
and we simply recover the SC algorithm from Section~\ref{subsec:sc} since $\Psi$ does not depend on the pairwise similarities~$\Sigmab$. Next, we present different structured sparsity-inducing penalties that yield more  effective algorithms.

\vsp
\subsubsection{Group-SC.}\label{subsec:groupsc}
For each location~$i$, the LSSC approach~\cite{mairal2009non} defines
groups of similar patches
$S_i \triangleq \left \{ j=1, \dots, n \: \text{s.t.} \:  \|\yb_i-\yb_j||_2^2 \leq \xi \right \}$ for some threshold $\xi$.
For computational reasons,
LSSC relaxes this definition in practice, and implements a clustering method
such that $S_i=S_j$ if $i$ and $j$ belong to the same group.
Then, under this clustering assumption and given a dictionary~$\Db$, LSSC minimizes
\begin{equation} \label{optim_pblm}
   \min_{\Ab} \frac{1}{2} \|\Yb^c-\Db \Ab\|_{\text{F}}^2 + \sum_{i=1}^N \Psi_i(\Ab) ~~\text{with}~~ \Psi_i(\Ab)\!=\!\lambda_i\|\Ab_i\|_{1,2},
\end{equation}
where $\Ab \!=\![\alphab_1,\ldots,\alphab_N]$ in $\Real^{m \times N}$ represents all codes, $\Ab_i\!=\![\alphab_l]_{l \in S_i}$,
$\|.\|_{1,2}$ is the group sparsity regularizer defined in~(\ref{groupeq}), $\|.\|_{\text{F}}$ is the Frobenius norm, $\Yb^c=[\yb_1^c,\ldots,\yb_N^c]$, and $\lambda_i$ depends on the group size.
As explained in Section~\ref{sec:related}, the role of the Group Lasso penalty is to encourage the codes $\alphab_j$ belonging to the same cluster to share the same sparsity pattern, see Figure~\ref{fig:sparse}.
For homogeneity reasons, we also consider the normalization factor $\lambda_i={\lambda}/{\sqrt{|S_i|}}$, as in~\cite{mairal2009non}.
Minimizing~(\ref{optim_pblm})  is easy with the ISTA method since we know how to compute the proximal operator of $\Psi$, which is described below:
\begin{lemma}[Proximal operator for the Group Lasso]
   Consider a matrix~$\Ub$ and call $\Zb=\prox_{\lambda\|.\|_{1,2}}[\Ub]$. Then, for all row $\Zb^j$ of $\Zb$,
   \begin{equation}
      \Zb^j = \max\left (1- \frac{ \lambda }{\|\Ub^j\|_2} ,0\right) \Ub^j.
   \end{equation}
\end{lemma}
Unfortunately, the procedure used to design the groups~$S_i$ does not yield a
differentiable relation between the denoised image~$\hat{\xb}$ and the
parameters to learn.  Therefore, we
relax the hard clustering assumption into a soft one, which is able to exploit
a similarity matrix~$\Sigmab$ representing pairwise relations between patches. Details about $\Sigmab$ are given in Section~\ref{sec:similarities}.
Yet, such a relaxation does not provide distinct groups of patches, preventing us from
using the Group Lasso penalty~(\ref{optim_pblm}).

This difficulty may be solved by introducing a joint relaxation of the Group Lasso penalty
and its proximal operator. First, we consider a similarity matrix~$\Sigmab$ that encodes the hard clustering assignment
used by LSSC---that is, $\Sigmab_{ij} = 1$ if $j$ is in~$S_i$ and~$0$ otherwise. Second, we note
that $\|\Ab_i\|_{1,2}=\|\Ab\diag(\Sigmab_i)\|_{1,2}$ where $\Sigmab_i$ is the $i$-th column of $\Sigmab$ that encodes
the $i$-th cluster membership.
Then, we adapt LISTA to problem~(\ref{optim_pblm}), with a different shrinkage parameter $\Lambdab^{(k)}_j$ per coordinate~$j$ and per iteration~$k$ as in Section~\ref{subsec:sc}, which yields
\begin{equation}
   \begin{split}
      \Bb & \leftarrow \Ab^{(k)} + \Cb^\top(\Yb^c-\Db\Ab^{(k)}) \\
      \Ab^{(k+1)}_{ij} & \leftarrow  \max\left (1- \frac{ \Lambda_j^{(k)} \sqrt{\|\Sigmab_i\|_1}}{\|(\Bb\diag(\Sigmab_i)^{\frac{1}{2}})^j\|_2} ,0\right) \Bb_{ij}, \\
   \end{split}\label{eq:lista_group}
\end{equation}
where the second update is performed for all $i,j$, the superscript $^j$ denotes the $j$-th row of a matrix, as above, and $\Ab_{ij}$ is simply the $j$-th entry of $\alphab_i$.

We are now in shape to relax the hard clustering assumption by allowing any
similarity matrix $\Sigmab$ in~(\ref{eq:lista_group}), leading to a relaxation of the Group Lasso penalty in Algorithm~\ref{alg:pseudo}. The resulting model is able to encourage similar patches to share similar sparsity patterns, while being trainable by minimization of the cost~(\ref{eq:cost}).


\subsection{Similarity Metrics}\label{sec:similarities}
We have computed similarities~$\Sigmab$ in various manners,
and implemented the following practical heuristics, which improve the computional complexity.

% \vsp
\paragraph{Online averaging of similarity matrices.}

As shown in Algorithm~\ref{alg:pseudo}, we use a convex combination of similarity matrices (using~$\nu_k$ in $[0,1]$, also learned by backpropagation),
which provides better results than computing the similarity on the current estimate only. This is expected since the current estimate~$\hat{\xb}$ may have lost too much signal information to compute accurately similarities,
whereas online averaging allows retaining information from the original signal.
We run an ablation study of our model reported in appendix to illustrate the need of similarity refinements during the iterations.
When they are no updates the model perfoms on average 0.15 dB lower than with 4 updates.

\vsp
\paragraph{Semi-local grouping.} As in all methods that exploit non-local self
similarities in images, we restrict the search for similar patches to $\yb_i$
to a window of size $w \times w$ centered around the patch. This approach is
commonly used to reduce the size of the similarity matrix and the global memory
cost of the method. This means that we will always have $\Sigmab_{ij}=0$ if pixels~$i$ and~$j$
are too far apart.

\vsp
\paragraph{Learned distance.}
We always use a similarity function of the
form~$\Sigmab_{ij}=e^{-{d_{ij}}}$, where $d_{ij}$ is a distance
between patches~$i$ and~$j$. As in classical deep learning models using non-local
approaches~\cite{liu2018non}, we do not directly use the $\ell_2$ distance
between patches.  Specifically, we consider
\begin{equation}
   d_{ij} = \|\diag(\kappab)(\hat{\xb}_i - \hat{\xb}_j)\|^2,
\end{equation}
where $\hat{\xb}_i$ and $\hat{\xb}_j$ are the $i$ and $j$-th patches from the current denoised image,
and $\kappab$ in $\Real^m$ is a set of weights, which are learned by backpropagation.

\subsection{Extension to Blind Denoising and Parameter Sharing}

The regularization parameter  $\lambda$  of Eq. (\ref{eq:l1_problem}) depends on the noise level.
In a blind denoising setting, it is possible to learn a shared set of dictionnaries $\{\Db,\Cb,\Wb\}$
and a set of different regularization parameters $\{\Lambda_{\sigma_0}, \dots, \Lambda_{\sigma_n} \}$ for various noise intensities.
At inference time, we use first a noise estimation algorithm from \cite{liu2013single} and then select the best regularization parameter to restore the image.


\subsection{Extension to Demosaicking}
\input{demosaicking.tex}

\subsection{Practical variants and implementation}\label{sec:extensions}
Finally, we discuss other practical variants
and implementation details.

\vsp
\paragraph{Dictionary initialization.}
A benefit of designing an architecture with a sparse coding
interpretation, is that the parameters $\Db,\Cb,\Wb$ can be initialized with a
classical dictionary learning approach, instead of using random weights, which
makes the initialization robust.  To do so, we use SPAMS toolbox
\cite{mairal2010online}.

\vsp
\paragraph{Block processing and dealing with border effects.}
The size of the tensor $\Sigmab$ grows quadratically with the image size, which
requires processing sequentially image blocks. % rather than the full image
Here, the block size is chosen to match the size~$w$ of the non local
window, which requires taking into account two important details:

(i) Pixels close to the image border belong to fewer patches than those
from the center, and thus receive less estimates in the averaging procedure.
When processing images per block, it is thus important to have a small overlap
between blocks, such that the number of estimates per pixel is consistent across the image.

(ii) We also process image blocks for training. It then is important to
take border effects into account, by rescaling the loss by the number of pixel estimates.





==> latexSource (copy)/related.tex <==

In this section, we introduce non-local sparse coding models for image denoising and present a differentiable algorithm for sparse coding~\cite{gregor2010learning}.

\vsp
\paragraph{Sparse coding models on learned dictionaries.}

A simple approach for image denoising introduced in~\cite{elad2006image} consists of assuming that
natural image patches can be well approximated by linear combinations
of few dictionary elements. Thus, a clean estimate of a noisy patch is obtained by computing a sparse approximation.
Given a noisy image, we denote by $\yb_1,\ldots,\yb_n$ the set of~$n$
overlapping patches of size $\sqrt{m} \times \sqrt{m}$, which we represent
by vectors in~$\Real^m$ for grayscale images. Each patch is then processed by
solving the sparse decomposition problem
\begin{equation}\label{eq:l1_problem}
   \min_{\alphab_i \in \Real^{p}} \frac{1}{2} \|\yb_i-\Db\alphab_i\|_2^2+\lambda\|\alphab_i\|_1,
\end{equation}
where $\Db=[\db_1,\ldots,\db_p]$ in $\Real^{m \times p}$ is the dictionary,
which we assume given at the moment, and $\|.\|_1$ is the $\ell_1$-norm, which is known to encourage
sparsity, see~\cite{mairal2014sparse}.
Note that a direct sparsity measure such as $\ell_0$-penalty may also be used,
at the cost of producing a combinatorially hard problem, whereas~(\ref{eq:l1_problem}) is convex.

Then, $\Db\alphab_i$ is a clean estimate of $\yb_i$. Since the patches overlap, we obtain
$m$ estimates for each pixel and the denoised image is obtained by averaging:
\begin{equation}
   \hat{\xb} = \frac{1}{m} \sum_{i=1}^n \Rb_i \Db \alphab_i, \label{eq:averaging}
\end{equation}
where $\Rb_i$ is a linear operator that places the patch $\Db \alphab_i$ at the position centered on pixel $i$ on the image.
Note that for simplicity, we neglect the fact that pixels close to the
image border admit less estimates, unless zero-padding is used.

Whereas we have previously assumed that a good dictionary~$\Db$ for natural images is
available, the authors of~\cite{elad2006image} have proposed
to learn $\Db$  by solving a matrix factorization
problem called \emph{dictionary learning}~\cite{field}.

\vsp
\paragraph{Differentiable algorithms for sparse coding.}
ISTA~\cite{figueiredo2003} is
a popular algorithm to solve problem~(\ref{eq:l1_problem}),
which alternates between gradient descent steps with respect to the smooth term of~(\ref{eq:l1_problem})
and the soft-thresholding operator $S_\eta(x)=  \sign(x) \max(0,|x| - \eta)$.

Note that such a step performs an affine transformation followed
by the pointwise non-linear function $S_{\eta}$, which makes it tempting to
consider $K$ steps of the algorithm, see it as a neural network with $K$
layers, and learn the corresponding weights.
Following such an insight, the authors of~\cite{gregor2010learning} have proposed the LISTA algorithm,
which is trained such that the resulting neural network learns to approximate the
solution of~(\ref{eq:l1_problem}).
Other variants were then proposed, see~\cite{chen2018theoretical,liu2018alista}; as~\cite{simon2019rethinking}, the one we have adopted may be written as
\begin{equation}
   \label{eq:recurrent}
   \alphab_i^{(k+1)} = S_{\Lambdab_{k}} \left [\alphab_i^{(k)}+ \Cb^\top\left(\yb_i-\Db\alphab_i^{(k)}\right) \right ],
\end{equation}
where $\Cb$ has the same size as $\Db$ and $\Lambdab_{k}$ in $\Real^p$ is such that
$S_{\Lambdab_{k}}$ performs a soft-thresholding operation with a
different threshold for each vector entry. Then,
the variables $\Cb, \Db$ and $\Lambdab_{k}$ are learned for a supervised image reconstruction task.

Note that when $\Cb = \eta\Db$ and $\Lambdab_{k}=\eta\lambda \ones$, where $\eta$ is a step size,
the recursion
recovers exactly the ISTA algorithm. Empirically, it has been observed that allowing
$\Cb \neq \Db$ accelerates convergence and could be
interpreted as learning a pre-conditioner for ISTA~\cite{liu2018alista}, whereas allowing
$\Lambdab_{k}$ to have entries different than~$\lambda \eta$ corresponds to using a weighted $\ell_1$-norm
and learning the weights.

There have been already a few attempts to leverage the LISTA algorithm  for specific  image restoration tasks such as
super-resolution~\cite{wang2015deep} or denoising~\cite{simon2019rethinking}, which we
extend in our paper with non-local priors and structured sparsity.

\vsp
\paragraph{Exploiting self-similarities.}
The non-local means approach \cite{buades2005non} consists of averaging similar patches
that are corrupted by i.i.d. zero-mean noise,
such that averaging reduces the noise variance without corrupting the signal.
The intuition relies on the fact that natural images
admit many local self-similarities. This is a non-parametric
approach (technically a Nadaraya-Watson estimator), which can be used to reduce the number of parameters of deep learning models.

\vsp
\paragraph{Non local sparse models.}
The LSSC approach~\cite{mairal2009non} relies on the principle of
joint sparsity.
Denoting by $S_i$ a set of patches similar to $\yb_i$ according to some criterion,

we consider the matrix
$\Ab_{i}=[\alphab_l]_{l \in S_i}$  in $\Real^{p\times |S_i|}$ of corresponding coefficients.
LSSC encourages the codes
$\{\alphab_l\}_{l \in S_i}$ to share the same sparsity pattern---that is, the set of non-zero entries.
This can be achieved by using a group-sparsity regularizer
\begin{equation}
   \label{groupeq}
   \|\Ab_i\|_{1,2} =   \sum_{j=1}^p \|\Ab_i^j\|_2,
\end{equation}
where $\Ab_i^j$ is the $j$-th row in $\Ab_i$.
The effect of this norm is to encourage sparsity patterns
to be shared across similar patches, as illustrated in Figure~\ref{fig:sparse}.
It may be seen as a convex relaxation of the number of non-zero rows in~$\Ab_i$, see~\cite{mairal2009non}.

Building a differentiable algorithm relying on both sparsity and non-local self-similarities
is challenging, as the clustering approach used by LSSC (or CSR) is typically not a continuous operation
of the dictionary parameters.

\begin{figure*}[t]
   \def \width{5.8}
   \centering
   \includegraphics[width=\width cm]{figures/sparse2.pdf}
   \label{fig:demos}
   \caption{(Left) sparsity pattern of codes with grey values representing non-zero entries; (right) group sparsity of codes for similar patches. Figure from \cite{mairal2009non}. }
   \label{fig:sparse}
\end{figure*}

\vsp
\paragraph{Deep learning models.}

In the context of image restoration, successful principles for deep learning models include very deep networks, batch norm, and residual learning~\cite{lefkimmiatis2018universal,zhang2017beyond,zhang2018ffdnet,zhang2019rnan}.  Recent models also use attention mechanisms to model self similarities, which are pooling operations akin to non-local means.
More precisely, a non local
module has been proposed in~\cite{liu2018non}, which performs weighed average
of similar features, and in \cite{plotz2018neural}, a relaxation
of the k-nearest selection rule is introduced for similar purposes.


\vsp
\paragraph{Model-based methods.}
Unfolding an optimization algorithm to design an inference architecture is not limited to sparse coding.
For instance \cite{sun2016deep,zhang2018ista} propose trainable architectures based on unrolled ADMM.
The authors of \cite{lefkimmiatis2017non,lefkimmiatis2018universal} propose a deep learning architecture
inspired from proximal gradient descent in order to solve a constrained optimization problem for denoising;
\cite{chen2016trainable} optimize hyperparameters of non linear reaction diffusion models; \cite{bertocchi2019deep}
unroll an interior point algorithm. Finally,  Plug-and-Play \cite{venkatakrishnan2013plug} is a framework for
image restoration exploiting a denoising prior as a modular part of model-based optimization methods to solve
various inverse problems. Several works leverage the plug-in principle with half quadratic spliting
\cite{zoran2011learning}, deep denoisers \cite{zhang2017learning}, message passing algorithms
\cite{fletcher2018plug}, or augmented Lagrangian \cite{romano2017little}.




==> latexSource (copy)/related_eccv.tex <==

In this section, we introduce non-local sparse coding models for image denoising and present a differentiable algorithm for sparse coding~\cite{gregor2010learning}, which we extend later.

\vsp
\paragraph{Sparse coding models on learned dictionaries.}
\vsp
\paragraph{Differentiable algorithms for sparse coding.}
\vsp
\paragraph{Exploiting non-local self-similarities.}

\vsp 
\paragraph{Non local sparse models.}

\vsp
\paragraph{Deep learning models.}


==> latexSource (copy)/ssim_tables.tex <==

\begin{table}[]
\footnotesize	
    \caption{\textbf{Blind denoising}. Training on BSD400. Performance is measured in terms of average PSNR. Best is in bold.}
    \centering
    \begin{tabular}{ccccccc}
    \toprule
    Noise level & CBM3D & DnCNN-B & CUNet & CUNLnet & SC\footnotemark & GroupSC   \\ \midrule
    params &-  & 666K & 93k & 93k & 116k  & 116k\\
    $\sigma=5$ & 40.24 & 40.11 & 40.31 & \underline{40.39} & - &  \textbf{40.62}\\
    $\sigma=10$  & 35.88 & 36.11& 36.08&\underline{36.20} &- &  \textbf{36.35}\\
    $\sigma=15$  & 33.49 & 33.88 & 33.78 & \underline{33.90}& {33.68} & \textbf{34.04}  \\
    $\sigma=20$  &31.88 & 32.36& 32.21& \underline{32.34}& - & \textbf{32.49}\\
    $\sigma=25$  & 30.68 & 21.22 & 31.03 & \underline{31.17} & - & \textbf{31.31} \\    \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table}

%\begin{table}[]
%\footnotesize	
%    \caption{\textbf{Blind denoising}. Training on BSD400. Performance is measured in terms of average PSNR. Best is in bold.}
%    \centering
%    \begin{tabular}{ccccccc}
%    \toprule
%    $\sigma$ & CBM3D & DnCNN-B & CUNet & CUNLnet & SC\footnotemark & GroupSC   \\ \midrule
%    params &-  & 666K & 196K & 196k & 121K  & 121k\\
%    5 & 40.24 & 40.11 & 40.31 & 40.39 & - & 39.98 \\
%    10 & 35.88 & 36.11& 36.08&36.20 &- & 36.18\\
%    15 & 33.49 & 33.88 & 33.78 & 33.90&  & 33.95 \\
%    20 &31.88 & 32.36& 32.21& 32.34& - & 32.43\\
%    25 & 30.68 & 21.22 & 31.03 & 31.17 & - & 31.31 \\   
%	30  &&&&&&   30.40\\
%    35 29.65\\
%    40 29.02\\
%    45  28.46\\
%    50&&&&27.89&&27.95\\
%    55 & 27.50\\
%     \bottomrule
%    \end{tabular}
%    \label{tab:my_label}
%\end{table}

\begin{table}[t] 
\footnotesize
	\centering
\caption{ \textbf{Color denoising} on CBSD68. Training on CBSD400 unless specified. Performance is measured in terms of average PSNR (in dB). Best is in bold.}\label{colour_table}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{Method}  & \multirow{2}{*}{Params} & \multicolumn{4}{c}{Noise level ($\sigma$)} \\
& & 5 & 15 & 25 & 50  \\
\midrule
\textit{Unsupervised} \\
CBM3D \cite{dabov2007image} &-& 40.24 &  33.49& 30.68&27.36\\
\midrule
% CUNLNet5 \cite{lefkimmiatis2018universal}&93k& 40.39 &33.90&31.17&27.89 \\
\textit{Trainable} \\
CSCnet \cite{simon2019rethinking} \footnotemark & 186k & - & 33.83 &31.18 &28.00 \\
NLNet\cite{lefkimmiatis2017non} &-& -&33.69 & 30.96 &27.64 \\
% IRCNN \cite{zhang2017learning}& && &33.86 &31.16& 27.86 \\
FFDNET \cite{zhang2018ffdnet} &486k & -&33.87 &31.21& 27.96 \\
% RNAN \cite{zhang2019rnan} & 7.5M &&36.60&&& \textbf{28.35} \\
CDnCNN  \cite{zhang2017beyond} & 668k & - & - &31.31 & -\\
\midrule
% \textbf{SC} (ours) &  63k  & &28.88& \\ 
% \textbf{CSR} (ours) & {68K}  &31.64  &  29.156 &26.08 \\
{SC} (baseline) & {112K} & {40.44} & {33.75} & 30.94 & 27.39  \\
{CSR} (ours) & {112K}& \underline{40.53} &\underline{34.05} & \underline{31.33} &   \underline{28.01}\\
%{GroupSC} \textit{speed} (ours)&{112K}&\textbf{40.58}&&\textbf{ 34.07} &\textbf{31.37}& &\textbf{-}  \\
{GroupSC} \textit{speed} (ours)&{118K}&\textbf{40.58}/0.9816&\textbf{34.11}/0.9353 &\textbf{31.44}/0.8917 &\textbf{28.05}/0.7974  \\
\bottomrule
\end{tabular}
	    \vspace*{-0.5cm}
\end{table}

\begin{table}[t] 
	\small
	\centering
	%\hspace*{-0.5cm}
	\caption{\textbf{Color denoising} on CBSD68. Training on BSD400.  Performance is measured in terms of average PSNR (in dB). Best is in bold.}\label{colour_table_rnan}
	\begin{tabular}{@{}lccccc@{}}
		\toprule
		Method  & Params &  $\sigma=10 $ & $\sigma=20$ & $\sigma=30$ & $\sigma=40$  \\
		\midrule
		RNAN \cite{zhang2019rnan} & 8.96M& \textbf{36.60} &  \textbf{30.73} \\
		{GroupSC} (ours)&{112K}& 36.40/0.9586& 32.58/0.9128 & 30.48 & 29.11/0.8329\\
		\bottomrule
	\end{tabular}
	    \vspace*{-0.5cm}

\end{table}

\footnotetext{CSCnet has been trained on a larger dataset made of 5214 images (waterloo + bsd432).}

\begin{table}[h]  
\small
\centering
\caption{\textbf{Grayscale Denoising} on BSD68. Training on BSD400 unless specified.  Performance is measured in terms of average PSNR (in dB). Best is in bold.}
% \label{tablenlrn}
\label{gray_table}
\begin{tabular}{@{}lccccc@{}}
\toprule
\multirow{2}{*}{Method}  & \multirow{2}{*}{Params} & \multicolumn{4}{c}{Noise Level ($\sigma$)} \\
& & 5 & 15 & 25 & 50 \\
\midrule
\textit{Unsupervised}\\
BM3D \cite{dabov2007image}&-&37.57 &31.07& 28.57&25.62\\
LSCC \cite{mairal2009non}&-&37.70&31.28&28.71 &25.72  \\
BM3D PCA \cite{dabov2009bm3d} & -&37.77 & 31.38  &28.82& 25.80\\
%WNNM \cite{gu2014weighted}& -& 37.76&31.37&28.83&25.87\\
 \midrule
 \textit{Trainable}\\
%   CSCnet \cite{simon2019rethinking}  \footnotemark[4]   &62k & 37.84 & 31.57 & { 29.11} & 26.24  \\
TNRD \cite{chen2016trainable}&- &- & 31.42 & 28.92 & 25.97 \\
CSCnet \cite{simon2019rethinking}  \footnotemark   &62k & 37.69 & 31.40 & { 28.93} & 26.04  \\
LKSVD & 45K & - & 31.54 & 29.07 & 26.13 \\
NLNet \cite{lefkimmiatis2017non}&-&- & 31.52 & 29.03 &26.07 \\
%UNLNet \cite{lefkimmiatis2017non}&-&37.62 & 31.47 & 28.96 &26.04 \\
FFDNet \cite{zhang2018ffdnet}& 486k&- & 31.63 & 29.19 &26.29 \\
DnCNN   \cite{zhang2017beyond}&556k & {37.68} &  \underline{31.73} & 29.22 & 26.23 \\
% N3   \cite{plotz2018neural}& 706k & \textbf{38.01} &  {31.79} & 29.30 & 26.39  \\
N3   \cite{plotz2018neural}& 706k & - &  - &  \underline{29.30} &  \underline{26.39}  \\
NLRN  \cite{liu2018non} & 330k& \underline{37.92} &\textbf{ 31.88} &\textbf{ 29.41} &\textbf{ 26.47}  \\
\midrule
{SC} (baseline)&  {68K}& 37.84 & 31.46&28.90&25.84 \\ 
{CSR} (ours)  & {68K}& 37.88  &31.64  &  29.16 &26.08 \\
{GroupSC} (ours)  & {68K}&\textbf{37.95}/0.9319 &31.71/0.8963 & 29.20/0.8336 & 26.17/0.7183 \\
\bottomrule
\end{tabular}
\vspace*{-0.5cm}
\end{table}


\footnotetext{We run here the model with the code provided by the authors online on the smaller training set BSD400.}
%
%\begin{table}[]
%\centering
%\scriptsize
%\begin{tabular}{lcccccccccccccc} \toprule
%\multicolumn{1}{l}{Method} & BM3D & LSCC & BM3D-PCA &CSCnet&CSCnet&NLNet& FFDNet & LKSVD & DnCNN & N3 & NLRN & SC & CSR & GroupSC\\ \midrule
%\multicolumn{1}{l}{Params} &  -    &      &         &      \\
%$\sigma=5$          &       37.57  & 37.70 & 37.77   & 37.84  & 37.69 & - & -   & -     & 37.68 &  -  & 37.92&37.84  & 37.88& 37.95  \\
%$\sigma=15$                         &      &      &         &      \\
%$\sigma=25$                         &      &      &         &      \\
%$\sigma=50$       &         25.62&      &      &         &       \\ \bottomrule
%\end{tabular}
%\end{table}

%\begin{table}[]
%\footnotesize
%    \centering
%    \begin{tabular}{ccccc}
%    \toprule
%    CLASSIC5 &jpeg & RNAN & sc & groupsc  \\
%    \midrule
%    qf = 10 & 27.82 & N/A  && 29.57\\
%    qf = 20 & 30.12 & 31.99 &&31.73\\
%    qf = 30 & 31.48 & N/A  &&33.02\\
%    qf = 40 & 32.43 & 34.03 &&33.88\\
%    \bottomrule
%    \end{tabular}
%    \caption{Jpeg artefact reduction. Training SR291}
%    \label{tab:jpeg}
%\end{table}



\begin{table}[t] \label{mosaic_table}
\centering

    \footnotesize	
    \caption{\textbf{Demosaicking}. Training on CBSD400. Performance is measured in terms of average PSNR/SSIM. Best is in bold.}
    \begin{tabular}{@{}llllll@{}}
    \toprule
    Method & Params & Kodak24 &BSD68 & Urban100 \\
    \midrule
    \textit{Unsupervised}\\
    LSCC        &  & 41.39 & 40.44 & 36.63\\
    \midrule
    \textit{Trainable}\\
    IRCNN (BSD400+Waterloo) &   &  40.54/0.9807   &39.96/0.9850& 36.64/0.9743 \\
    Kokinos \cite{kokkinos2018deep} (MIT dataset ) & 380k &    41.5   & -& - \\
    MMNet \cite{kokkinos2019iterative} (MIT dataset ) & 380k & 42.0 & - & -\\
    RNAN \cite{zhang2019rnan} (CBSD400) & {8.96M} &  \textbf{42.86}  & \underline{42.61} & - \\
    \midrule
    %{SC} (BSD400)   (ours) & 118k & 0.67 & 42.34 & 41.88 & 37.50\\ 
   % {GroupSC \textit{speed}} (BSD400)   (ours) &  {118k} &{2.39}  &  42.63 & 42.81 &  38.13 \\
    {GroupSC} (CBSD400)  (ours) &  {118k}  &  \underline{42.71}/0.9901 & \textbf{42.91}/0.9938 & \textbf{38.21}/0.9804 \\ 
    \bottomrule
    \end{tabular}
    \vspace*{-0.5cm}

\end{table}


\footnotetext{We report here our scores without any cropping similarly to \cite{zhang2019rnan}. If we crop 10 pixels from the border following \cite{zhang2017learning} we obtain a score of \textbf{??} db on Kodak24 and \textbf{??} db on BSD68.}




%\begin{table}[]
%    \centering
%    \begin{tabular}{cccccc}
%    \toprule
%        Model  &  Params & s = 50 & s=\red{25} & s= \red{10}  \\ \midrule
%        RNAN & 8.96M & 2.35 (42.61)\\
%        GroupSC  & 118K&  2.39 & 8.60 & 43.03\\     \bottomrule
%
%    \end{tabular}
%    \caption{\red{recalc inf times} Inference time demosaicking. eval BSD68}
%    \label{tab:speed_modaic}
%\end{table}

==> latexSource (copy)/supp_mat.tex <==

\subsection{Proof of propostion \ref{csr_prox}}
The proximal operator of the function $\Psi_i(\ub) = \| \ub \|_1 + \gamma \| \ub - \betab_i \|_1$  for $\ub$ in~$\Real^p$ is defined as
\begin{equation*} \label{prox_psi}
    \prox_{\lambda \Psi_i} [\zb]=  \argmin_{\ub \in \Real^p} \frac{1}{2}\|\zb-\ub\|^2 + \lambda \|\ub\|_1 + \lambda \gamma \| \ub - \betab_i\|_1
\end{equation*}
The optimality condition for the previous problem is
$$ 0 \in \triangledown (\frac{1}{2} || \zb - \ub ||_2^2) + \partial (\lambda ||\ub||_1) + \partial (\lambda \gamma ||\ub - \betab_i||_1) $$
$$\Leftrightarrow 0 \in \ub - \zb + \lambda \partial ||\ub||_1 + \lambda \gamma  \partial ||\ub - \betab_i||_1  $$
We consider each component separately. We suppose that $\betab_i[j] \neq 0$, otherwise  $\Psi_i(\ub)[j]$ boils down to the $\ell_1$ norm. And we also suppose $\lambda,\gamma >0$.

Let's examine the first case where $u[j] = 0$. The subdifferential of the $\ell_1$ norm is the interval $[-1,1]$ and the optimality condition is
\begin{align*}
    0 \in \ub[j] - \zb[j] + [-\lambda,\lambda] + \lambda \gamma \sign(\ub[j]-\betab_i[j]) \\
    \Leftrightarrow \zb[j] \in [-\lambda,\lambda] -  \lambda \gamma \sign(\betab_i[j])
\end{align*}
Similarly if $\ub[j] = \betab_i[j]$
\begin{equation*}
    \zb[j] \in \betab_i[j] + \lambda \sign(\betab_i[j]) + [-\lambda \gamma,\lambda \gamma] 
\end{equation*}


Finally let's examine the case where $u[j] \neq 0$ and $u[j] \neq \betab_i[j]$: then, $\partial ||\ub||_1 = \sign(\ub[j])$ and $\partial ||\ub - \betab_i||_1 = \sign(\ub[j] - \betab_i[j])$. The minimum $u[j]^*$ is obtained as 
\begin{align*}
     0 = \ub[j] - \zb[j] + \lambda \sign(\ub[j]) + \lambda \gamma \sign(\ub[j]-\betab_i[j]) \\
     \Leftrightarrow \ub[j]^* =  \zb[j] - \lambda \sign(\ub[j]^*) - \lambda \gamma \sign(\ub[j]^*-\betab_i[j]) 
\end{align*}

We study separately the cases where $\ub[j]>\betab[j]$, $0<\ub[j]<\betab[j]$ and $\ub[j]<0$ when $\betab_i[j]>0$ and proceed similarly when $\betab_i<0$. With elementary operations we can derive the expression of $\zb[j]$ for each case. Putting the cases all together we obtain the formula.

 
\subsection{Additional experimental details}


In order to accelerate the inference time of the non-local models, we update patch similarities every $1/f$ steps. Where $f$ is the frequency of the correlation updates.
We summarize in Table \ref{hyperparam} the set of hyperparameters that we selected for the experiments reported in the main tables.
We selected the same hyper-parameters for the baselines, except that we do not compute pairwise patch similarities.

\begin{table}[h]
    \small
    \centering
    \caption{Hyper-parameters of our experiments.}
        \label{hyperparam}
    \begin{tabular}{lccc}
    \toprule
    Experiment & Color d. & Gray d. & Demosaicking \\
    \midrule
    Patch size & 7 & 9 & 9 \\
    Dictionnary size  &256 & 256 & 256 \\
    Nr epochs  & 300  &  300 & 200 \\
    Batch size &  25 & 25 & 16 \\
    $K$ iterations  & 24 & 24 & 24 \\
    \begin{tabular}[c]{@{}l@{}}Correlation update\\ frequency $f$\end{tabular} & ${1}/{6}$ & ${1}/{6}$ &  ${1}/{6}$ \\
    \bottomrule
    \end{tabular}

\end{table}
    
    
\subsection{Influence of patch and dictionnary size}

We investigate in Table \ref{ablation_table} the influence of two hyperparameters: the patch size and the dictionnary size for grayscale image denoising. For this experiment we run  a lighter version of the model groupSC, in order to accelerate the training. The batch size was decreased from 25 to 16, the frequency of the correlation updates was decreased from $1/6$ to $1/8$ and the intermediate patches are not approximated with averaging.  These changes accelerate the training but lead to slightly lower performances when compared with the model trained in the standard setting. It explains the gap between the scores in Table ~\ref{ablation_table} and in Table~\ref{gray_table}.

\begin{table}[h]
    \small
    \centering
    \caption{Influence of the dictionnary size and the patch size on the denoising performance. Grayscale denoising on BSD68. Models are trained on BSD400. Models are trained in a light setting to accelerate the training.}
    \label{ablation_table}
    \begin{tabular}{clccc}
        \toprule
        Noise ($\sigma$) &   Patch size   & n=128 & n=256 & 512   \\ 
        \midrule
        \multirow{3}{*}{$5$} 
        & k=7 &  37.91     &  37.92     & -     \\
        & k=9 &  37.90     & 37.92        &   37.96    \\
        & k=11 &  37.89     &  37.89      & -        \\
        \midrule
        \multirow{3}{*}{$15$} 
        & k=7 &   31.60    &  31.63       & -       \\
        & k=9 &   31.62    &31.67      & 31.71       \\
        & k=11 & 31.63  &  31.67      & -        \\
        \midrule
        \multirow{3}{*}{$25$}
        & k=7 &   29.10    & 29.11        & -       \\
        & k=9 &  29.12     & 29.17      &  29.20    \\
        & k=11 &  29.13     & 29.18      &-       \\
        \bottomrule
    \end{tabular}
\end{table}  

\subsection{Grayscale denoising: evaluation on multiple datasets}
We provide additional grayscale denoising results on other datasets in term of PSNR of our model in Table \ref{gray_app}.
\begin{table}[h]
\small
\centering
\caption{Grayscale denoising on different datasets.Training on BSD400.  Performance is measured in terms of average PSNR (in dB). }
\label{gray_app}
\begin{tabular}{cccccc}
    \toprule
    Dataset                   & Noise & BM3D  & DnCnn & NLRN  & {GroupSC} \\ 
    \midrule
    \multirow{4}{*}{\textbf{Set12}}   
        & 5    &  - &-&  -    &  38.40    \\
    & 15    & 32.37 & 32.86 & 33.16 & 32.85      \\
    & 25    & 29.97 & 30.44 & 30.80 &  30.44    \\
    & 50    & 26.72 & 27.18 & 27.64 &  27.14    \\
    \midrule
    \multirow{4}{*}{\textbf{BSD68}}    & 5  &  37.57&  37.68&  {37.92}     &  37.95    \\
    & 15    & 31.07 & 31.73 & 31.88 &   31.70   \\
    & 25    & 28.57 & 29.23 & 29.41 &   29.20   \\
    & 50    & 25.62 & 26.23 & 26.47 &  26.18    \\
    \midrule
    \multirow{4}{*}{\textbf{Urban100}}
    & 5     &   -    &    -  &    -   &  38.51    \\
    & 15    & 32.35 & 32.68 & 33.45 &   32.71   \\
    & 25    & 29.70 & 29.91 & 30.94 &  30.05    \\
    & 50    & 25.95 & 26.28 & 27.49 &  26.44  \\ \bottomrule
\end{tabular}
\end{table}


\subsection{Color denoising: evaluation on multiple datasets}
We provide additional color denoising results on other datasets in term of PSNR of our model in Table~\ref{color_app}.
\begin{table}[] 
    \small
    \centering
    \caption{Color denoising on different datasets.Training on CBSD400.  Performance is measured in terms of average PSNR (in dB). }
    \label{color_app}
    \begin{tabular}{cccc}
        \toprule 	
    Dataset                   & Noise& CBM3D & {GroupSC} \\ 	\midrule
    \multirow{4}{*}{\textbf{Kodak24}}   
    & 5   & -  &       40.72    \\
    & 15  &  33.25       &    34.98     \\
    & 25  &  32.06  &   32.44     \\
    &  50 &  28.75  &       29.16    \\
\midrule	\multirow{4}{*}{\textbf{CBSD68}}
    & 5  & 40.24  & 40.61     \\
    & 15 & 33.49  &  34.10    \\
    & 25 & 30.68 &  31.42    \\
    & 50 & 27.36 &  28.03   \\
\midrule	\multirow{4}{*}{\textbf{Urban100}} 
    &  5  & -         &  39.74 \\
    &  15  &    33.22     & 34.11  \\
    &  25  &   30.59     &  31.63   \\
    &  50  &   26.59     & 28.20    \\ 	\bottomrule
    \end{tabular}
\end{table}




==> latexSource (copy)/tables_main.tex <==

\begin{table}[tb]
%\vspace*{-1cm}
\footnotesize	
    \caption{\textbf{Blind denoising} on CBSD68, training on CBSD400. Performance is measured in terms of average PSNR. 
    SSIMs are in the appendix. 
    Best is in bold, second is underlined.}\label{tab:blind}
    \centering
    \begin{tabular}{ccccccc}
    \toprule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Noise\\level\end{tabular}} & CBM3D\cite{dabov2009bm3d} & CDnCNN-B \cite{zhang2017beyond} & CUNet\cite{lefkimmiatis2018universal} & CUNLnet\cite{lefkimmiatis2018universal} & SC (ours) & GroupSC (ours)  \\ 
     &-  & 666k & 93k & 93k & 115k  & 115k\\ \midrule
    5 & 40.24 & 40.11 & 40.31 & \underline{40.39} & 40.30 &  \textbf{40.43}\\
    10  & 35.88 & 36.11& 36.08&\underline{36.20} & 36.07 &  \textbf{36.29}\\
    15 & 33.49 & 33.88 & 33.78 & \underline{33.90}& {33.72} & \textbf{34.01}  \\
     20 &31.88 & \underline{32.36} & 32.21& {32.34}& 32.11& \textbf{32.41}\\
     25& 30.68 & \underline{31.22} & 31.03 & 31.17 & 30.91 & \textbf{31.25} \\    \bottomrule
    \end{tabular}
    % \vspace*{-0.5cm}

    \label{tab:my_label}
\end{table}


\begin{table}[tb]
\footnotesize
	\centering
   \caption{ \textbf{Color denoising} on CBSD68, training on CBSD400 for all methods except CSCnet (Waterloo+CBSD400). 
   Performance is measured in terms of average PSNR. SSIMs are reported in the appendix.}\label{colour_table}
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\multirow{2}{*}{Method} &\multirow{2}{*}{Trainable } & \multirow{2}{*}{Params} & \multicolumn{4}{c}{Noise level ($\sigma$)} \\
& & & 5 & 10 & 15 & 25 & 30 & 50  \\
\midrule
%\textit{Unsupervised} \\
CBM3D \cite{dabov2007image} & \xmark &-& 40.24 & - & 33.49& 30.68&-&27.36\\
\midrule
%\textit{Trainable} \\
   CSCnet \cite{simon2019rethinking} &  & 186k & - &- &33.83 &31.18 &-&28.00 \\
CNLNet\cite{lefkimmiatis2017non}&  &-& -&-&33.69 & 30.96& - &27.64 \\
FFDNET \cite{zhang2018ffdnet}&  &486k & -&-&33.87 &31.21& - &27.96 \\
% RNAN \cite{zhang2019rnan} & 7.5M &&36.60&&& \textbf{28.35} \\
CDnCNN  \cite{zhang2017beyond}&  & 668k & 40.50 & 36.31 & 33.99 &31.31& -& 28.01\\
RNAN \cite{zhang2019rnan}&  & 8.96M &-& \textbf{36.60}&- & -&\textbf{30.73}&\textbf{28.35} \\
\midrule

{SC} (baseline) & & {119k} & {40.44}& - & {33.75} & 30.94 & - &27.39  \\
% {CSR} (ours) & & {119k}& {40.53} & - &{34.05} & {31.33} & - & {28.01}\\
%{GroupSC} \textit{speed} (ours)&{112K}&\textbf{40.58}&&\textbf{ 34.07} &\textbf{31.37}& &\textbf{-}  \\
{GroupSC} (ours)& &{119k}&\underline{40.58}& \underline{36.40} &\underline{34.11} &\underline{31.44} & \underline{30.58} &\underline{28.05}  \\
\bottomrule
\end{tabular}
	    % \vspace*{-0.5cm}
\end{table}



\begin{table}[tb]
\small
\centering
\caption{\textbf{Grayscale Denoising} on BSD68, training on BSD400 for all methods except CSCnet (Waterloo+BSD400).  
Performance is measured in terms of average PSNR.
SSIMs are reported in the appendix.}
% \label{tablenlrn}
\label{gray_table}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{Method}  & \multirow{2}{*}{Trainable} & \multirow{2}{*}{Params}   & \multicolumn{4}{c}{Noise Level ($\sigma$)} \\
& & & 5 & 15 & 25 & 50 \\
\midrule
%\textit{Unsupervised}\\
BM3D \cite{dabov2007image}& \xmark &-&37.57 &31.07& 28.57&25.62\\
LSSC \cite{mairal2009non}& \xmark &-&37.70&31.28&28.71 &25.72  \\
BM3D PCA \cite{dabov2009bm3d}& \xmark  & -&37.77 & 31.38  &28.82& 25.80\\
%WNNM \cite{gu2014weighted}& -& 37.76&31.37&28.83&25.87\\
 \midrule
% \textit{Trainable}\\
 TNRD \cite{chen2016trainable}&  &- &- & 31.42 & 28.92 & 25.97 \\
CSCnet \cite{simon2019rethinking} &  &62k & 37.84 & 31.57 & { 29.11} & 26.24  \\
   CSCnet(BSD400) \cite{simon2019rethinking}\footnotemark[2]  &  &62k & 37.69 & 31.40 & { 28.93} & 26.04  \\
   LKSVD~\cite{scetbon2019deep} &  & 45K & - & 31.54 & 29.07 & 26.13 \\
NLNet \cite{lefkimmiatis2017non}& & -&- & 31.52 & 29.03 &26.07 \\
%UNLNet \cite{lefkimmiatis2017non}&-&37.62 & 31.47 & 28.96 &26.04 \\
FFDNet \cite{zhang2018ffdnet}&  & 486k&- & 31.63 & 29.19 &26.29 \\
DnCNN   \cite{zhang2017beyond}&  &556k & {37.68} &  \underline{31.73} & 29.22 & 26.23 \\
% N3   \cite{plotz2018neural}& 706k & \textbf{38.01} &  {31.79} & 29.30 & 26.39  \\
N3   \cite{plotz2018neural}&  & 706k & - &  - &  \underline{29.30} &  \underline{26.39}  \\
NLRN  \cite{liu2018non} &  & 330k& \underline{37.92} &\textbf{ 31.88} &\textbf{ 29.41} &\textbf{ 26.47}  \\
\midrule
{SC} (baseline)& &  {68k}& 37.84 & 31.46&28.90&25.84 \\ 
% {CSR} (ours)&   & {68k}& 37.88  &31.64  &  29.16 &26.08 \\
{GroupSC} (ours)&   & {68k}&\textbf{37.95}&31.71& 29.20& 26.17 \\
\bottomrule
\end{tabular}
%\vspace*{-0.5cm}
\end{table}


\begin{table}

    \caption{ \textbf{Jpeg artefact reduction} on Classic5 with training on CBSD400. 
    Performance is measured in terms of average PSNR. 
    SSIMs are reported in the appendix.}
\footnotesize
    \centering
    \begin{tabular}{cccccccc}
    \toprule
    \begin{tabular}[c]{@{}c@{}}Quality\\ factor\end{tabular} &jpeg & SA-DCT \cite{foi2007pointwise} & AR-CNN \cite{yu2016deep} & TNRD\cite{chen2016trainable} & DnCNN-3 \cite{zhang2017beyond} & SC & GroupSC  \\
    \midrule
    qf = 10 &  27.82 & 28.88 &29.04 & 29.28 &\underline{29.40} & 29.39& \textbf{29.61}\\
    qf = 20 &  30.12 & 30.92 &31.16 & 30.12& \underline{31.63} & {31.58} &\textbf{31.78}\\
    qf = 30 & 31.48  & 32.14 &32.52 & 31.47 & \underline{32.91}  &  {32.80} &\textbf{33.06}  \\
    qf = 40 & 32.43  & 33.00 &33.34 & - &\underline{33.75} & 33.75&\textbf{33.91}\\
    \bottomrule
    \end{tabular}
    \label{tab:jpeg}
\end{table}
\footnotetext{We run here the model with the code provided by the authors online on the smaller training set BSD400.}


\begin{table} \label{mosaic_table}
\centering

    \footnotesize	
    \caption{\textbf{Demosaicking.} Training on CBSD400 unless a larger dataset is specified between parenthesis.
     Performance is measured in terms of average PSNR. SSIMs are reported in the appendix.}
    \begin{tabular}{@{}lccccc@{}}
    \toprule
    Method &Trainable & Params & Kodak24 &BSD68 & Urban100 \\
    \midrule
    %\textit{Unsupervised}\\
    LSSC     & \xmark   &  - & 41.39 & 40.44 & 36.63\\
    \midrule
   % \textit{Trainable}\\
    IRCNN \cite{zhang2017learning} (BSD400+Waterloo \cite{ma2016waterloo})&   & -  &  40.54  &39.9& 36.64 \\
    Kokinos \cite{kokkinos2018deep} (MIT dataset \cite{gharbi2016deep}) & & 380k &    41.5   & -& - \\
    MMNet \cite{kokkinos2019iterative} (MIT dataset \cite{gharbi2016deep})&  & 380k & 42.0 & - & -\\
    RNAN \cite{zhang2019rnan}&  & {8.96M} &  \textbf{42.86}  & \underline{42.61} & - \\
    \midrule
    {SC} (ours)&  & 119k& 42.34 & 41.88 & 37.50\\ 

    {GroupSC}   (ours)&  &  {119k}  &  \underline{42.71}& \textbf{42.91} & \textbf{38.21} \\ 
    \bottomrule
    \end{tabular}

\end{table}

==> latexSource (copy)/teaser.tex <==
\begin{figure*}[t]
\def \width{2.3}
\def \2{14}
\def \1{23}
\def \2{14}
\def \3{07}
\def \4{20}

\def \width{2.0}
\def \Width{2.0}

\centering
\def \width{2.3}
\def \2{14}
\def \1{23}
\def \2{14}
\def \3{07}
\def \4{20}
% \def \width{2.3}
% \def \Width{2.3}
\def \width{2.3}
\def \Width{2.3}

\centering
\begin{tabular}{ccccccc}
\includegraphics[width=\width cm]{figures/mosa/70_sc.png} & 
\includegraphics[width=\width cm]{figures/mosa/60_sc.png} &
%\includegraphics[width=\width cm]{figures/mosa/66_sc.png} &
\includegraphics[width=\Width cm]{figures/tease/23_sc.png}&
\includegraphics[width=\Width cm]{figures/tease/g11_sc.png}&
\includegraphics[width=\width cm]{figures/jpeg/23_sc.png} &


\\
\includegraphics[width=\width cm]{figures/mosa/70_group.png} & 
\includegraphics[width=\width cm]{figures/mosa/60_group.png}&
%\includegraphics[width=\width cm]{figures/mosa/66_group.png}&
\includegraphics[width=\Width cm]{figures/tease/23_group.png} &
\includegraphics[width=\Width cm]{figures/tease/g11_group.png}&
\includegraphics[width=\width cm]{figures/jpeg/23_group.png} & 

 \\


\multicolumn{2}{c}{Demosaicking} & \multicolumn{2}{c}{Denoising} & Jpeg deblocking   \\

\end{tabular}
\caption{Effect of combining sparse and non-local priors for different reconstruction tasks. Top: reconstructions with sparse prior only, exhibiting artefacts. Bottom: reconstruction with both priors, artefact-free. Best seen in color by zooming on a computer screen.}
\label{fig:mosaic}
\vspace*{-0.2cm}
\end{figure*}


==> related_eccv.tex <==

In this section, we introduce non-local sparse coding models for image denoising and present a differentiable algorithm for sparse coding~\cite{gregor2010learning}, which we extend later.

\vsp
\paragraph{Sparse coding models on learned dictionaries.}
\vsp
\paragraph{Differentiable algorithms for sparse coding.}
\vsp
\paragraph{Exploiting non-local self-similarities.}

\vsp 
\paragraph{Non local sparse models.}

\vsp
\paragraph{Deep learning models.}


==> ssim_tables.tex <==

\begin{table}[]
\footnotesize	
    \caption{\textbf{Blind denoising}. Training on BSD400. Performance is measured in terms of average PSNR. Best is in bold.}
    \centering
    \begin{tabular}{ccccccc}
    \toprule
    Noise level & CBM3D & DnCNN-B & CUNet & CUNLnet & SC\footnotemark & GroupSC   \\ \midrule
    params &-  & 666K & 93k & 93k & 116k  & 116k\\
    $\sigma=5$ & 40.24 & 40.11 & 40.31 & \underline{40.39} & - &  \textbf{40.62}\\
    $\sigma=10$  & 35.88 & 36.11& 36.08&\underline{36.20} &- &  \textbf{36.35}\\
    $\sigma=15$  & 33.49 & 33.88 & 33.78 & \underline{33.90}& {33.68} & \textbf{34.04}  \\
    $\sigma=20$  &31.88 & 32.36& 32.21& \underline{32.34}& - & \textbf{32.49}\\
    $\sigma=25$  & 30.68 & 21.22 & 31.03 & \underline{31.17} & - & \textbf{31.31} \\    \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table}

%\begin{table}[]
%\footnotesize	
%    \caption{\textbf{Blind denoising}. Training on BSD400. Performance is measured in terms of average PSNR. Best is in bold.}
%    \centering
%    \begin{tabular}{ccccccc}
%    \toprule
%    $\sigma$ & CBM3D & DnCNN-B & CUNet & CUNLnet & SC\footnotemark & GroupSC   \\ \midrule
%    params &-  & 666K & 196K & 196k & 121K  & 121k\\
%    5 & 40.24 & 40.11 & 40.31 & 40.39 & - & 39.98 \\
%    10 & 35.88 & 36.11& 36.08&36.20 &- & 36.18\\
%    15 & 33.49 & 33.88 & 33.78 & 33.90&  & 33.95 \\
%    20 &31.88 & 32.36& 32.21& 32.34& - & 32.43\\
%    25 & 30.68 & 21.22 & 31.03 & 31.17 & - & 31.31 \\   
%	30  &&&&&&   30.40\\
%    35 29.65\\
%    40 29.02\\
%    45  28.46\\
%    50&&&&27.89&&27.95\\
%    55 & 27.50\\
%     \bottomrule
%    \end{tabular}
%    \label{tab:my_label}
%\end{table}

\begin{table}[t] 
\footnotesize
	\centering
\caption{ \textbf{Color denoising} on CBSD68. Training on CBSD400 unless specified. Performance is measured in terms of average PSNR (in dB). Best is in bold.}\label{colour_table}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{Method}  & \multirow{2}{*}{Params} & \multicolumn{4}{c}{Noise level ($\sigma$)} \\
& & 5 & 15 & 25 & 50  \\
\midrule
\textit{Unsupervised} \\
CBM3D \cite{dabov2007image} &-& 40.24 &  33.49& 30.68&27.36\\
\midrule
% CUNLNet5 \cite{lefkimmiatis2018universal}&93k& 40.39 &33.90&31.17&27.89 \\
\textit{Trainable} \\
CSCnet \cite{simon2019rethinking} \footnotemark & 186k & - & 33.83 &31.18 &28.00 \\
NLNet\cite{lefkimmiatis2017non} &-& -&33.69 & 30.96 &27.64 \\
% IRCNN \cite{zhang2017learning}& && &33.86 &31.16& 27.86 \\
FFDNET \cite{zhang2018ffdnet} &486k & -&33.87 &31.21& 27.96 \\
% RNAN \cite{zhang2019rnan} & 7.5M &&36.60&&& \textbf{28.35} \\
CDnCNN  \cite{zhang2017beyond} & 668k & - & - &31.31 & -\\
\midrule
% \textbf{SC} (ours) &  63k  & &28.88& \\ 
% \textbf{CSR} (ours) & {68K}  &31.64  &  29.156 &26.08 \\
{SC} (baseline) & {112K} & {40.44} & {33.75} & 30.94 & 27.39  \\
{CSR} (ours) & {112K}& \underline{40.53} &\underline{34.05} & \underline{31.33} &   \underline{28.01}\\
%{GroupSC} \textit{speed} (ours)&{112K}&\textbf{40.58}&&\textbf{ 34.07} &\textbf{31.37}& &\textbf{-}  \\
{GroupSC} \textit{speed} (ours)&{118K}&\textbf{40.58}/0.9816&\textbf{34.11}/0.9353 &\textbf{31.44}/0.8917 &\textbf{28.05}/0.7974  \\
\bottomrule
\end{tabular}
	    \vspace*{-0.5cm}
\end{table}

\begin{table}[t] 
	\small
	\centering
	%\hspace*{-0.5cm}
	\caption{\textbf{Color denoising} on CBSD68. Training on BSD400.  Performance is measured in terms of average PSNR (in dB). Best is in bold.}\label{colour_table_rnan}
	\begin{tabular}{@{}lccccc@{}}
		\toprule
		Method  & Params &  $\sigma=10 $ & $\sigma=20$ & $\sigma=30$ & $\sigma=40$  \\
		\midrule
		RNAN \cite{zhang2019rnan} & 8.96M& \textbf{36.60} &  \textbf{30.73} \\
		{GroupSC} (ours)&{112K}& 36.40/0.9586& 32.58/0.9128 & 30.48 & 29.11/0.8329\\
		\bottomrule
	\end{tabular}
	    \vspace*{-0.5cm}

\end{table}

\footnotetext{CSCnet has been trained on a larger dataset made of 5214 images (waterloo + bsd432).}

\begin{table}[h]  
\small
\centering
\caption{\textbf{Grayscale Denoising} on BSD68. Training on BSD400 unless specified.  Performance is measured in terms of average PSNR (in dB). Best is in bold.}
% \label{tablenlrn}
\label{gray_table}
\begin{tabular}{@{}lccccc@{}}
\toprule
\multirow{2}{*}{Method}  & \multirow{2}{*}{Params} & \multicolumn{4}{c}{Noise Level ($\sigma$)} \\
& & 5 & 15 & 25 & 50 \\
\midrule
\textit{Unsupervised}\\
BM3D \cite{dabov2007image}&-&37.57 &31.07& 28.57&25.62\\
LSCC \cite{mairal2009non}&-&37.70&31.28&28.71 &25.72  \\
BM3D PCA \cite{dabov2009bm3d} & -&37.77 & 31.38  &28.82& 25.80\\
%WNNM \cite{gu2014weighted}& -& 37.76&31.37&28.83&25.87\\
 \midrule
 \textit{Trainable}\\
%   CSCnet \cite{simon2019rethinking}  \footnotemark[4]   &62k & 37.84 & 31.57 & { 29.11} & 26.24  \\
TNRD \cite{chen2016trainable}&- &- & 31.42 & 28.92 & 25.97 \\
CSCnet \cite{simon2019rethinking}  \footnotemark   &62k & 37.69 & 31.40 & { 28.93} & 26.04  \\
LKSVD & 45K & - & 31.54 & 29.07 & 26.13 \\
NLNet \cite{lefkimmiatis2017non}&-&- & 31.52 & 29.03 &26.07 \\
%UNLNet \cite{lefkimmiatis2017non}&-&37.62 & 31.47 & 28.96 &26.04 \\
FFDNet \cite{zhang2018ffdnet}& 486k&- & 31.63 & 29.19 &26.29 \\
DnCNN   \cite{zhang2017beyond}&556k & {37.68} &  \underline{31.73} & 29.22 & 26.23 \\
% N3   \cite{plotz2018neural}& 706k & \textbf{38.01} &  {31.79} & 29.30 & 26.39  \\
N3   \cite{plotz2018neural}& 706k & - &  - &  \underline{29.30} &  \underline{26.39}  \\
NLRN  \cite{liu2018non} & 330k& \underline{37.92} &\textbf{ 31.88} &\textbf{ 29.41} &\textbf{ 26.47}  \\
\midrule
{SC} (baseline)&  {68K}& 37.84 & 31.46&28.90&25.84 \\ 
{CSR} (ours)  & {68K}& 37.88  &31.64  &  29.16 &26.08 \\
{GroupSC} (ours)  & {68K}&\textbf{37.95}/0.9319 &31.71/0.8963 & 29.20/0.8336 & 26.17/0.7183 \\
\bottomrule
\end{tabular}
\vspace*{-0.5cm}
\end{table}


\footnotetext{We run here the model with the code provided by the authors online on the smaller training set BSD400.}
%
%\begin{table}[]
%\centering
%\scriptsize
%\begin{tabular}{lcccccccccccccc} \toprule
%\multicolumn{1}{l}{Method} & BM3D & LSCC & BM3D-PCA &CSCnet&CSCnet&NLNet& FFDNet & LKSVD & DnCNN & N3 & NLRN & SC & CSR & GroupSC\\ \midrule
%\multicolumn{1}{l}{Params} &  -    &      &         &      \\
%$\sigma=5$          &       37.57  & 37.70 & 37.77   & 37.84  & 37.69 & - & -   & -     & 37.68 &  -  & 37.92&37.84  & 37.88& 37.95  \\
%$\sigma=15$                         &      &      &         &      \\
%$\sigma=25$                         &      &      &         &      \\
%$\sigma=50$       &         25.62&      &      &         &       \\ \bottomrule
%\end{tabular}
%\end{table}

%\begin{table}[]
%\footnotesize
%    \centering
%    \begin{tabular}{ccccc}
%    \toprule
%    CLASSIC5 &jpeg & RNAN & sc & groupsc  \\
%    \midrule
%    qf = 10 & 27.82 & N/A  && 29.57\\
%    qf = 20 & 30.12 & 31.99 &&31.73\\
%    qf = 30 & 31.48 & N/A  &&33.02\\
%    qf = 40 & 32.43 & 34.03 &&33.88\\
%    \bottomrule
%    \end{tabular}
%    \caption{Jpeg artefact reduction. Training SR291}
%    \label{tab:jpeg}
%\end{table}



\begin{table}[t] \label{mosaic_table}
\centering

    \footnotesize	
    \caption{\textbf{Demosaicking}. Training on CBSD400. Performance is measured in terms of average PSNR/SSIM. Best is in bold.}
    \begin{tabular}{@{}llllll@{}}
    \toprule
    Method & Params & Kodak24 &BSD68 & Urban100 \\
    \midrule
    \textit{Unsupervised}\\
    LSCC        &  & 41.39 & 40.44 & 36.63\\
    \midrule
    \textit{Trainable}\\
    IRCNN (BSD400+Waterloo) &   &  40.54/0.9807   &39.96/0.9850& 36.64/0.9743 \\
    Kokinos \cite{kokkinos2018deep} (MIT dataset ) & 380k &    41.5   & -& - \\
    MMNet \cite{kokkinos2019iterative} (MIT dataset ) & 380k & 42.0 & - & -\\
    RNAN \cite{zhang2019rnan} (CBSD400) & {8.96M} &  \textbf{42.86}  & \underline{42.61} & - \\
    \midrule
    %{SC} (BSD400)   (ours) & 118k & 0.67 & 42.34 & 41.88 & 37.50\\ 
   % {GroupSC \textit{speed}} (BSD400)   (ours) &  {118k} &{2.39}  &  42.63 & 42.81 &  38.13 \\
    {GroupSC} (CBSD400)  (ours) &  {118k}  &  \underline{42.71}/0.9901 & \textbf{42.91}/0.9938 & \textbf{38.21}/0.9804 \\ 
    \bottomrule
    \end{tabular}
    \vspace*{-0.5cm}

\end{table}


\footnotetext{We report here our scores without any cropping similarly to \cite{zhang2019rnan}. If we crop 10 pixels from the border following \cite{zhang2017learning} we obtain a score of \textbf{??} db on Kodak24 and \textbf{??} db on BSD68.}




%\begin{table}[]
%    \centering
%    \begin{tabular}{cccccc}
%    \toprule
%        Model  &  Params & s = 50 & s=\red{25} & s= \red{10}  \\ \midrule
%        RNAN & 8.96M & 2.35 (42.61)\\
%        GroupSC  & 118K&  2.39 & 8.60 & 43.03\\     \bottomrule
%
%    \end{tabular}
%    \caption{\red{recalc inf times} Inference time demosaicking. eval BSD68}
%    \label{tab:speed_modaic}
%\end{table}

==> supp_mat.tex <==

\subsection{Proof of propostion \ref{csr_prox}}
The proximal operator of the function $\Psi_i(\ub) = \| \ub \|_1 + \gamma \| \ub - \betab_i \|_1$  for $\ub$ in~$\Real^p$ is defined as
\begin{equation*} \label{prox_psi}
    \prox_{\lambda \Psi_i} [\zb]=  \argmin_{\ub \in \Real^p} \frac{1}{2}\|\zb-\ub\|^2 + \lambda \|\ub\|_1 + \lambda \gamma \| \ub - \betab_i\|_1
\end{equation*}
The optimality condition for the previous problem is
$$ 0 \in \triangledown (\frac{1}{2} || \zb - \ub ||_2^2) + \partial (\lambda ||\ub||_1) + \partial (\lambda \gamma ||\ub - \betab_i||_1) $$
$$\Leftrightarrow 0 \in \ub - \zb + \lambda \partial ||\ub||_1 + \lambda \gamma  \partial ||\ub - \betab_i||_1  $$
We consider each component separately. We suppose that $\betab_i[j] \neq 0$, otherwise  $\Psi_i(\ub)[j]$ boils down to the $\ell_1$ norm. And we also suppose $\lambda,\gamma >0$.

Let's examine the first case where $u[j] = 0$. The subdifferential of the $\ell_1$ norm is the interval $[-1,1]$ and the optimality condition is
\begin{align*}
    0 \in \ub[j] - \zb[j] + [-\lambda,\lambda] + \lambda \gamma \sign(\ub[j]-\betab_i[j]) \\
    \Leftrightarrow \zb[j] \in [-\lambda,\lambda] -  \lambda \gamma \sign(\betab_i[j])
\end{align*}
Similarly if $\ub[j] = \betab_i[j]$
\begin{equation*}
    \zb[j] \in \betab_i[j] + \lambda \sign(\betab_i[j]) + [-\lambda \gamma,\lambda \gamma] 
\end{equation*}


Finally let's examine the case where $u[j] \neq 0$ and $u[j] \neq \betab_i[j]$: then, $\partial ||\ub||_1 = \sign(\ub[j])$ and $\partial ||\ub - \betab_i||_1 = \sign(\ub[j] - \betab_i[j])$. The minimum $u[j]^*$ is obtained as 
\begin{align*}
     0 = \ub[j] - \zb[j] + \lambda \sign(\ub[j]) + \lambda \gamma \sign(\ub[j]-\betab_i[j]) \\
     \Leftrightarrow \ub[j]^* =  \zb[j] - \lambda \sign(\ub[j]^*) - \lambda \gamma \sign(\ub[j]^*-\betab_i[j]) 
\end{align*}

We study separately the cases where $\ub[j]>\betab[j]$, $0<\ub[j]<\betab[j]$ and $\ub[j]<0$ when $\betab_i[j]>0$ and proceed similarly when $\betab_i<0$. With elementary operations we can derive the expression of $\zb[j]$ for each case. Putting the cases all together we obtain the formula.

 
\subsection{Additional experimental details}


In order to accelerate the inference time of the non-local models, we update patch similarities every $1/f$ steps. Where $f$ is the frequency of the correlation updates.
We summarize in Table \ref{hyperparam} the set of hyperparameters that we selected for the experiments reported in the main tables.
We selected the same hyper-parameters for the baselines, except that we do not compute pairwise patch similarities.

\begin{table}[h]
    \small
    \centering
    \caption{Hyper-parameters of our experiments.}
        \label{hyperparam}
    \begin{tabular}{lccc}
    \toprule
    Experiment & Color d. & Gray d. & Demosaicking \\
    \midrule
    Patch size & 7 & 9 & 9 \\
    Dictionnary size  &256 & 256 & 256 \\
    Nr epochs  & 300  &  300 & 200 \\
    Batch size &  25 & 25 & 16 \\
    $K$ iterations  & 24 & 24 & 24 \\
    \begin{tabular}[c]{@{}l@{}}Correlation update\\ frequency $f$\end{tabular} & ${1}/{6}$ & ${1}/{6}$ &  ${1}/{6}$ \\
    \bottomrule
    \end{tabular}

\end{table}
    
    
\subsection{Influence of patch and dictionnary size}

We investigate in Table \ref{ablation_table} the influence of two hyperparameters: the patch size and the dictionnary size for grayscale image denoising. For this experiment we run  a lighter version of the model groupSC, in order to accelerate the training. The batch size was decreased from 25 to 16, the frequency of the correlation updates was decreased from $1/6$ to $1/8$ and the intermediate patches are not approximated with averaging.  These changes accelerate the training but lead to slightly lower performances when compared with the model trained in the standard setting. It explains the gap between the scores in Table ~\ref{ablation_table} and in Table~\ref{gray_table}.

\begin{table}[h]
    \small
    \centering
    \caption{Influence of the dictionnary size and the patch size on the denoising performance. Grayscale denoising on BSD68. Models are trained on BSD400. Models are trained in a light setting to accelerate the training.}
    \label{ablation_table}
    \begin{tabular}{clccc}
        \toprule
        Noise ($\sigma$) &   Patch size   & n=128 & n=256 & 512   \\ 
        \midrule
        \multirow{3}{*}{$5$} 
        & k=7 &  37.91     &  37.92     & -     \\
        & k=9 &  37.90     & 37.92        &   37.96    \\
        & k=11 &  37.89     &  37.89      & -        \\
        \midrule
        \multirow{3}{*}{$15$} 
        & k=7 &   31.60    &  31.63       & -       \\
        & k=9 &   31.62    &31.67      & 31.71       \\
        & k=11 & 31.63  &  31.67      & -        \\
        \midrule
        \multirow{3}{*}{$25$}
        & k=7 &   29.10    & 29.11        & -       \\
        & k=9 &  29.12     & 29.17      &  29.20    \\
        & k=11 &  29.13     & 29.18      &-       \\
        \bottomrule
    \end{tabular}
\end{table}  

\subsection{Grayscale denoising: evaluation on multiple datasets}
We provide additional grayscale denoising results on other datasets in term of PSNR of our model in Table \ref{gray_app}.
\begin{table}[h]
\small
\centering
\caption{Grayscale denoising on different datasets.Training on BSD400.  Performance is measured in terms of average PSNR (in dB). }
\label{gray_app}
\begin{tabular}{cccccc}
    \toprule
    Dataset                   & Noise & BM3D  & DnCnn & NLRN  & {GroupSC} \\ 
    \midrule
    \multirow{4}{*}{\textbf{Set12}}   
        & 5    &  - &-&  -    &  38.40    \\
    & 15    & 32.37 & 32.86 & 33.16 & 32.85      \\
    & 25    & 29.97 & 30.44 & 30.80 &  30.44    \\
    & 50    & 26.72 & 27.18 & 27.64 &  27.14    \\
    \midrule
    \multirow{4}{*}{\textbf{BSD68}}    & 5  &  37.57&  37.68&  {37.92}     &  37.95    \\
    & 15    & 31.07 & 31.73 & 31.88 &   31.70   \\
    & 25    & 28.57 & 29.23 & 29.41 &   29.20   \\
    & 50    & 25.62 & 26.23 & 26.47 &  26.18    \\
    \midrule
    \multirow{4}{*}{\textbf{Urban100}}
    & 5     &   -    &    -  &    -   &  38.51    \\
    & 15    & 32.35 & 32.68 & 33.45 &   32.71   \\
    & 25    & 29.70 & 29.91 & 30.94 &  30.05    \\
    & 50    & 25.95 & 26.28 & 27.49 &  26.44  \\ \bottomrule
\end{tabular}
\end{table}


\subsection{Color denoising: evaluation on multiple datasets}
We provide additional color denoising results on other datasets in term of PSNR of our model in Table~\ref{color_app}.
\begin{table}[] 
    \small
    \centering
    \caption{Color denoising on different datasets.Training on CBSD400.  Performance is measured in terms of average PSNR (in dB). }
    \label{color_app}
    \begin{tabular}{cccc}
        \toprule 	
    Dataset                   & Noise& CBM3D & {GroupSC} \\ 	\midrule
    \multirow{4}{*}{\textbf{Kodak24}}   
    & 5   & -  &       40.72    \\
    & 15  &  33.25       &    34.98     \\
    & 25  &  32.06  &   32.44     \\
    &  50 &  28.75  &       29.16    \\
\midrule	\multirow{4}{*}{\textbf{CBSD68}}
    & 5  & 40.24  & 40.61     \\
    & 15 & 33.49  &  34.10    \\
    & 25 & 30.68 &  31.42    \\
    & 50 & 27.36 &  28.03   \\
\midrule	\multirow{4}{*}{\textbf{Urban100}} 
    &  5  & -         &  39.74 \\
    &  15  &    33.22     & 34.11  \\
    &  25  &   30.59     &  31.63   \\
    &  50  &   26.59     & 28.20    \\ 	\bottomrule
    \end{tabular}
\end{table}



